Incrementally Verifiable Oracle Aided Computation

Incrementally verifiable computation (IVC) allows a prover to maintain a short proof that can be efficiently updated after each computation step, without retaining or recomputing the preceding execution. Standard IVC schemes do not directly address a crucial feature of AI tasks: their dependence on external information and expertise. We construct IVC schemes for oracle-aided computations under the LWE assumption by first constructing SNARGs, and then extending them to IVC. We consider the following two settings, where below, k is the security parameter, n is the input length, and T, S, and Q are the time, space, and oracle-query bounds. 1. Robust computations: For bounded-space computations, including non-deterministic computations, in which every accepting purported execution on a false input contains at least an eps-fraction of incorrect oracle answers, we construct privately verifiable SNARGs and IVC. Public parameters, private verification keys, and proofs have length poly(k ,S, log T,1/eps), and verification uses O(k/eps) oracle calls. We complement this result with a lower bound ruling out (deterministic) publicly verifiable SNARGs and IVCs with public parameters of length o(n), and o(Q) verifier oracle queries. 2. Signed oracles: For oracles that digitally sign their query-answer pairs, we construct publicly verifiable SNARGs and IVC without a robustness assumption, and with oracle-free setup and verification. Public parameters and proofs have length poly(k,S,log T). For deterministic computations with oracle query and answer lengths poly(k,log T), we remove the dependence on S, obtaining public parameter and proof lengths poly(k,log T). All our constructions have adaptive completeness and soundness.

==> 0.5-camera-ready-abstract.tex <==
\begin{abstract}
We construct a succinct non-interactive argument (SNARG) system for every NP language $\mathcal{L}$ that has a propositional proof of {\em non-membership}, i.e. of $x\notin \mathcal{L}$. The soundness of our SNARG system relies on the hardness of the learning with errors (LWE) problem.  The common reference string (CRS) in our construction grows with the \emph{space} required to verify the propositional proof, and the size of the proof grows \emph{poly-logarithmically in the length} of the propositional proof.

Unlike most of the literature on SNARGs, our result implies SNARGs for languages $\mathcal L$ with proof length shorter than logarithmic in the deterministic time complexity of $\mathcal L$. Our SNARG improves over prior SNARGs for such ``hard'' NP languages (Sahai and Waters, STOC 2014, Jain and Jin, FOCS 2022) in several ways:

1) For languages with \emph{polynomial-length} propositional proofs of non-membership, our SNARGs are based on a single, \emph{polynomial-time} falsifiable assumption, namely LWE. 

2) Our construction handles \emph{super-polynomial length} propositional proofs, as long as they have bounded space, under the subexponential LWE assumption. 

3) Our SNARGs have a \emph{transparent setup}, meaning that no private randomness is required to generate the CRS. 

Moreover, our approach departs dramatically from these prior works: we show how to design SNARGs for hard languages without publishing a program (in the CRS) that has the power to verify $\mathsf{NP}$ witnesses. 

The key new idea in our construction is what we call a ``locally unsatisfiable extension'' of the $\mathsf{NP}$ verification circuit $\{C_x\}_x$. We say that an $\mathsf{NP}$ verifier has a locally unsatisfiable extension if for every $x\not\in \mathcal L$, there exists an extension $E_x$ of $C_x$ that is not even \emph{locally satisfiable} in the sense of a local assignment generator [Paneth-Rothblum, TCC 2017]. Crucially, we allow $E_x$ to be depend arbitrarily on $x$ rather than being efficiently constructible.

In this work, we show -- via a ``hash-and-BARG'' for a hidden, encrypted computation -- how to build SNARGs for all languages with locally unsatisfiable extensions. We additionally show that propositional proofs of unsatisfiability generically imply the existence of locally unsatisfiable extensions, which allows us to deduce our main results.

As an illustrative example, our results imply a SNARG for the decisional Diffie-Hellman (DDH) language under the LWE assumption.
\end{abstract}


==> 1-camera-ready-intro.tex <==
 \section{Introduction}
\label{sec:intro}

Succinct non-interactive arguments ($\mathsf{SNARG}$s) are a powerful cryptographic primitive whose feasibility is still poorly understood. Informally, a $\SNARG$ for an $\mathsf{NP}$ language $\cL$ is a computationally sound non-interactive argument system for $\cL$ whose proofs are short, much shorter than the length of an $\mathsf{NP}$ witness, and easy to verify. To achieve this, the prover and the verifier are given access to a common reference string $\crs$ (also called a structured random string), and this string is used both to produce the $\SNARG$ proofs and to verify them.  

In the random oracle model, it is known that there are $\SNARG$s for \emph{every} $\mathsf{NP}$ language \cite{STOC:Kilian92,FOCS:Micali94}. However, constructing $\SNARG$s for $\NP$ in the ``plain model" under falsifiable and preferably standard cryptographic assumptions remains a widely open problem.  Indeed, Gentry and Wichs~\cite{STOC:GenWic11} formalized a serious barrier to constructing $\SNARG$s in the case where the cheating prover is allowed to choose the statement $x$ adaptively based on the $\crs$; such a soundness guarantee is known as {\em adaptive soundness}.  

Faced with the Gentry-Wichs barrier, we focus on the problem of constructing $\SNARG$s with {\em non-adaptive soundness}, where cheating provers are restricted to choose the statement~$x$ independently of the $\crs$.  Non-adaptive soundness is interesting for two reasons:  First, in many settings (1) the adversary indeed does not get to choose the statement depending on the $\crs$, or (2) one can informally argue that statements that do depend on the $\crs$ are likely to be contrived.  Moreover, by using standard complexity-leveraging techniques, one can obtain adaptive soundness from non-adaptive soundness, at the price of making the $\SNARG$ proof grow with the input size, which is often much smaller than the witness size.
%\vnote{Shouldn't one first explain why non-adaptive soundness is a {\em meaningful / useful} goal? The text below says why it's hard, but there are lots of hard things that are useless / not worth doing.} \ynote{Done}
\paragraph{$\SNARG$s vs. Proofs of non-Membership.} Let us first describe why even constructing such \emph{non-adaptive} $\SNARG$s for all of $\NP$ seems to be challenging, by giving an intuitive barrier to constructing computationally sound argument systems that applies to most known $\SNARG$ constructions \cite{STOC:KalRazRot14,STOC:BraHolKal17,STOC:BKKSW18,FOCS:ChoJaiJin21,TCC:KalVaiZha21,C:BBKLP23}.  

Soundness of a $\SNARG$ is typically proved by exhibiting a polynomial (or sub-exponential) time reduction~$R$ that uses any cheating prover $P^*$, in a black-box way, to break the underlying (falsifiable) cryptographic assumption.  In the case of non-adaptive soundness, the analysis fixes any $x\notin \cL$ and presents a reduction $R_x$ that uses any successful cheating prover $P^*_x$ 
%that generates an accepting $\SNARG$ for the (false) claim ``$x\in \cL$'' 
to break the assumption. Intuitively, such an $R_x$ together with the mathematical proof $\pi_x$, that indeed $R_x$ can use any successful $P^*_x$ to break the underlying assumption,  constitutes a  ``witness'' for $x\notin \cL$.  Note that for $x\in \cL$, such a pair $(R_x,\pi_x)$ does not exist (unless the underlying assumption is false), since for $x\in \cL$ there does exist an {\em efficient} convincing prover $P_x$ (who is given a corresponding witness $w$), and thus there does not exist a poly-time reduction $R_x$ that uses $P_x$ to break the assumption (unless, of course, the assumption is false). We  believe that there are $\NP$ languages for which membership for  $x\in \overline{\cL}$ requires a ``witness'' of size $2^{|x|}$, and thus we believe that any such reduction $R_x$ ``must be'' of exponential size, which in turn implies that we need to rely on a cryptographic assumption that is $2^{|x|}$-secure.  Indeed, the only known $\SNARG$ construction for all of $\NP$ which is based on falsifiable assumptions, due to Sahai and Waters~\cite{STOC:SahWat14}, uses a reduction of size $2^{|x|}$ and thus relies on a $2^{|x|}$-hard cryptographic assumption. 

We note that the above intuitive argument is not a proof.\footnote{A proof of soundness is a single proof $\pi$ for the statement that for every $x\notin \cL$, the reduction $R_x$ can be used to break the assumption, whereas the above argument assumes that for every $x\notin \cL$ there is a pair $(R_x,\pi_x)$ where $\pi_x$ is a (mathematical) proof that $R_x$ can use any successful prover to break the underlying assumption.
It is not clear that one can convert the proof~$\pi$ into a polynomial size proof $\pi_x$ for every $x\notin \cL$.  Indeed, if the underlying $\SNARG$ has statistical soundness then%one cannot necessarily convert the mathematical proof $\pi$ into a ``per $x$'' mathematical proof $\pi_x$, since in the statistical setting,
~$R_x$ can simply be empty, and the proof $\pi$ can be trivial. Nevertheless, it turns out that most known $\SNARG$ constructions can be seen as producing a subexponential-length proof $\pi_x$.} Nevertheless, this thought experiment strongly suggests a connection between constructing $\SNARG$s for an $\mathsf{NP}$ language $\mathcal L$ and the problem of \emph{mathematically proving} that an instance $x$ is in the language $\overline{\cL}$. 
We thus focus on the following informal question: 

%\ynote{changed this sentence} That said, we believe that for all $\SNARG$ constructions in the literature that are not statistically sound (and are not indistinguishable from being statistically sound),  the mathematical proof $\pi$ can be converted into an efficient ``per $x$'' mathematical proof $\pi_x$.

%Nevertheless, for $\SNARG$s that do not have statistical soundness it seems natural that one would be able to convert a uniform~$\pi$ into $\pi_x$ for every $x\notin \cL$.  The reason is that in this setting,  $R_x$ cannot be trivial and always refuse to break the assumption. The proof $\pi$ that argues that $R_x$ breaks the assumption can be seen as a ``proof''

%Indeed we believe that it can be done for all $\SNARG$ constructions in the literature (that rely on falsifiable assumptions).

%Intuitively, for this proof strategy to work the reduction $R_x$ must ``know" that $x$ is not in $\cL$, since if $x\in\cL$ then $R_x$ would not succeed in breaking the assumption given access to any $P^*_x$ (since there is an efficient such prover). However, if $R_x$ ``knows" that $x\notin \cL$ then there must be a proof that $x\notin \cL$. 
% \ynote{Better?} \vnote{Why is this last statement true? This seems to assume that $\cL \in \mathsf{coNP}$ which we haven't said anything about so far.}\znote{Agree, how about the following story: We don't know how to build SNARGs for NP due to Gentry-Wichs. Even with iO [SW14], the CRS is long. So we ask can we build SNARGs for some interesting subclasses of NP? Then we say we observe that in many applications of SNARGs, the specific language we are considering has more structures, (e.g. the DDH language, we can non-adaptively ``know'' the discrete log for any fixed instance), those structures allow us to know ``why $x \notin L$'' for every fixed $x \notin L$ and hence provide more information than brute-forcely enumerating all possible NP-witness. Hence, in this work, we aim to explore if we can use such ``why'' to get around GW and build SNARGs). Naturally, this ``why'' can be formalized as math proofs, and the most fundamental form of math proof is propositional logic...} 

\begin{quote}
\begin{center} Are there non-adaptive $\SNARG$s for every language $\cL\in \NP$ with a security \\ reduction of size~$\poly(T)$, where $T$ is the length of a proof for $x\notin \cL$?
\end{center}
\end{quote}






\subsection{Our Results}

In this work, we provide a positive answer for the case where the size-$T$ proof for $x\notin \cL$ is a (extended Frege) {\em propositional proof} \cite{krajicek95}.  Our $\SNARG$ proof length grows {\em poly-logarithmically} with $T$, while the $\crs$ grows linearly with the {\em space} required to verify this propositional proof, and non-adaptive soundness relies on the $\poly(T)$-hardness of $\LWE$. In the case that the propositional proof is of polynomial size (and the instance size is polynomially related to the security parameter) the assumption becomes the polynomial hardness of $\LWE$.


\begin{theorem}[Informal]\label{thm:main-intro}
Given functions $T=T(n)$ and $S=S(n)$, there exists a $\SNARG$ for any $\NP$ language~$\cL$ such that every $x\notin \cL$ has a propositional proof for $x\notin \cL$ of length~$T=T(|x|)$, that can be verified in space $S=S(|x|)$. The size of the $\CRS$ is $S\cdot\poly(\secp)$ and the size of the $\SNARG$ is $\poly(\secp,\log T)$. The $\SNARG$ is non-adaptively sound based on the $T$-hardness of $\LWE$.
\end{theorem}
Two remarks about \Cref{thm:main-intro} are in order.
%: the first should be interpreted as a strength of the theorem and the second as a weakness.  
First, the $\SNARG$ construction does not depend on the propositional proof, rather only on the parameters $T$ and $S$. The actual propositional proof appears only in the analysis. Thus, one does not need to ``know'' such a propositional proof in order to construct the $\SNARG$, nor does such a proof need to be efficiently computable.

Second, we consider the implications of \Cref{thm:main-intro} when $T(n)$ is polynomial in $n$.  In this setting, we get a $\SNARG$ under the polynomial hardness of $\LWE$ for a subclass of $\NP\cap \coNP$, namely ones that have a poly-size {\em propositional proof} for $x\notin L$.  
While it is tempting to think that languages in $\mathsf{NP}\cap \mathsf{coNP}$ should have propositional proofs of non-membership, it is not necessarily the case. 

\iffalse 
Denoting by $M$ the non-deterministic Turing machine corresponding to $\cL$ and by $\bar{M}$ the one corresponding to $\bar{\cL}$, one may hope to convert the tableau of the non-deterministic Turing machine $\bar{M}$ that proves that $x\notin \cL$ into a poly-size propositional proof for $x\notin \cL$.
Unfortunately, it is not clear that this can be done. One can convert the tableau for $\bar{M}(x,\bar{w})=1$ into a poly-size propositional proof of this fact. However, this is insufficient.  One needs to add a propositional proof that the existence of $\bar{w}$ such that $\bar{M}(x,\bar{w})=1$ implies that for every $w$ it holds that $M(x,w)=0$.  It is not clear that every language $\cL\in \NP\cap \coNP$ has an efficient propositional proof of this latter fact.
\fi 

\iffalse Second, we note that \Cref{thm:main-intro} is interesting also for a polynomial ~$T(n)$.  In this setting we get a $\SNARG$ under the polynomial hardness of $\LWE$ for a subclass of $\NP\cap \coNP$.
We emphasize that it does not give a $\SNARG$ for all languages in $\NP\cap \coNP$, but rather only for those for which there is a poly-size {\em propositional proof} for $x\notin L$.  
While it is tempting to think that one can efficiently convert a proof of non-membership into a propositional proof, it is not necessarily the case. 
Denoting by $M$ the non-deterministic Turing machine corresponding to $\cL$ and by $\bar{M}$ the one corresponding to $\bar{\cL}$, one may hope to convert the tableau of the non-deterministic Turing machine $\bar{M}$ that proves that $x\notin \cL$ into a poly-size propositional proof for $x\notin \cL$.
Unfortunately, it is not clear that this can be done. One can convert the tableau for $\bar{M}(x,\bar{w})=1$ into a poly-size propositional proof of this fact. However, this is insufficient.  One needs to add a propositional proof that the existence of $\bar{w}$ such that $\bar{M}(x,\bar{w})=1$ implies that for every $w$ it holds that $M(x,w)=0$.  It is not clear that every language $\cL\in \NP\cap \coNP$ has an efficient propositional proof of this latter fact.
\fi 

Nevertheless, important languages in $\NP \cap \coNP$ \emph{do} have such proofs. As an example, we observe that the $\DDH$ language does have a poly-size propositional proof of non-membership.  We thus obtain the following corollary.

\begin{corollary}\label{cor:DDH}
    There is a $\SNARG$ for the $\DDH$ language that has non-adaptive soundness under the polynomial hardness of $\LWE$.  The proof length is $\poly(\secp)$ and the $\crs$ length is $\poly(n,\secp)$, where $n$ is the instance size.
\end{corollary}

One interesting fact about \Cref{cor:DDH} is that the $\DDH$ language does not appear to have a {\em non-signaling $\PCP$} (with small locality). Indeed, it is believed that the $\DDH$ language, on groups of size roughly $2^n$, are not decidable in $\mathsf{DTIME}(2^{n^\epsilon})$ for some constant $\epsilon > 0$. As a result, our $\SNARG$ has proof length which is \emph{less than logarithmic} in the deterministic time complexity of the language! This stands in contrast to (1) most prior works on $\SNARG$s from standard assumptions, which were only for languages that have non-signaling PCPs,\footnote{The only other work that break this non-signaling barrier are the works of \cite{STOC:SahWat14,FOCS:JaiJin22} which rely on indistinguishability obfuscation, and the recent work \cite{C:BBKLP23}.  We elaborate on all these three works, and compare them to our work, in \Cref{sec:related}.} and (2) the Gentry-Wichs barrier, which says that exactly this kind of $\SNARG$ with adaptive soundness is impossible to achieve.   We believe that the techniques we use in this work to circumvent these barriers are of independent interest and will lead to further follow-up work.

%Indeed, we believe that our new techniques, which we elaborate on below, are of independent interest and will find more applications.

% We then show how to shorten the $\crs$, to avoid the $\NP\cap \coNP$ limitation.  We define the notion of the {\em space} of a propositional proof,\footnote{We defer the precise definition of space to \Cref{sec:super-poly-EF}.}  and prove the following more general theorem.

% \begin{theorem}[Informal]\label{thm:intro:EF-super-poly}
% For every functions $\ell=\ell(n)$ and $s=s(n)$, we construct a $\SNARG$ and prove that it has non-adaptive soundness under $\LWE$ for any $\NP$ language $\cL$ for which for every $x\notin \cL$ there is a propositional proof for $x\notin \cL$ of length~$\ell=\ell(|x|)$ and space $s=s(|x|)$. The size of the $\CRS$ is $s\cdot\poly(\secp)$ and the size of the $\SNARG$ is $\poly(\secp,\log \ell)$.
% \end{theorem}

%We note that this theorem gives us $\SNARG$s for languages outside of $\NP\cap\coNP$ since the length of the propositional proof can be super-polynomial, as long as the space needed to verify it is polynomial. More specifically, it gives a $\SNARG$ only for languages in $\NP\cap\mathsf{DTISP}(T,S)$,\footnote{$\mathsf{DTISP}(T,S)$ is the set of languages that can be determined by a time-$T$ and space-$S$ deterministic Turing machine.} \vnote{Is it DTISP or NTISP? The space is used to verify, not generate, the co-witness, right?}\znote{I think this should be coNISP?} where the $\crs$ size grows linearly with the space~$S$ and the $\SNARG$ grows logarithmically with the time~$T$.  As was mentioned previously, we do not get such a $\SNARG$ for every language in $\NP\cap\mathsf{DTISP}(T,S)$, rather only for those for which there is a $\poly(T)$ size and $\poly(S)$ space {\em propositional proof} that $\bar{M}(x)=1$ implies that for every $w$, $M(x,w)=0$, where as above, $M$ is the non-deterministic Turing machine corresponding to $\cL$ and $\bar{M}$ is the deterministic time-$T$ and space-$S$ Turing machine corresponding to $\bar{\cL}$.




\paragraph{Encrypt-Hash-and-$\BARG$}
We propose a new method for constructing $\SNARG$s.
Specifically, we extend the Hash-and-$\BARG$ method \cite{FOCS:ChoJaiJin21,TCC:KalVaiZha21} to an ``encrypt-hash-and-$\BARG$'' method.  We elaborate on this method in \Cref{sec:techniques}, and in what follows we state its implications.  

For a given $\NP$ language $\cL$ and for any instance $x\in\{0,1\}^*$, we denote by $C_x$ the verification circuit that given an input $w$ outputs~$1$ if and only if $w$ is a valid witness for $x\in\cL$.

\begin{theorem}[informal, see the full version]\label{thm:intro:ext-poly}
For every parameter $\ell=\ell(n)$, we construct a $\SNARG$ for any $\NP$ language $\cL$ that has the following property:  For every $x\notin \cL$ there exists an extension~$E_x$ of the verification circuit~$C_x$ such that $E_x$ has the property that local consistency with locality $\ell$ implies global correctness. The length of the $\SNARG$ is $\poly(\secp,\ell,\log{|E_x|})$, and the length of the $\crs$ is $|E_x|\cdot \poly(\secp)$.\footnote{In fact, we can even compress the $\crs$ length to polynomial in a succinct description $\aux_x$ of the circuit $E_x$, which may be much smaller.}  The $\SNARG$ has non-adaptive soundness assuming the $|E_x|$-hardness of $\LWE$.
\end{theorem}

We call such a family of circuits $\{E_x\}$ a \emph{locally unsatisfiable extension} of the circuit $C(x, w)$. We emphasize that in \Cref{thm:intro:ext-poly}, the extended circuit $E_x$ need not be efficiently computable from $x$, which is how we circumvent prior barriers.  Our $\SNARG$ construction does not use this extension and it is only used in the analysis.
\ynote{In particular, one can use our $\SNARG$ for {\em any} $\NP$ language, even an $\NP$ complete one.  If a cheating prover can break soundness then this implies that this circuit does not have a locally unsatisfiable extension, something that currently we do not know how to prove.}





Moreover, we show an improved version of \cref{thm:intro:ext-poly} that holds even when the extended circuit $E_x$ has super-polynomial size, provided that every \emph{gate} of $E_x$ can be computed by a polynomial-size sub-circuit. % show that the $\crs$ need not grow with the description of the entire extension $\langle{E_x\rangle}$. Instead, we can make the $\crs$ grow linearly with $\gamma(n)$ which is defined so that for every gate $g$ in $E_x$ the the sub-circuit of $E_x$ computing $g$ is of size at most $\gamma(|x|)$.\footnote{One could strengthen this result to make the $\crs$ grow only with the (possibly succinct) description of the circuit computing each gate~$g$.  For the sake of simplicity we chose to avoid this extra layer of complication in the technical section.}  

\begin{theorem}[informal, see the full version]\label{thm:intro:ext-super-poly}
For parameters $\ell=\ell(n)$ and $\gamma=\gamma(n)$, there exists a $\SNARG$ for any $\NP$ language $\cL$ that has the following two properties: (1) For every $x\notin \cL$ there exists an extension~$E_x$ of the verification circuit~$C_x$ such that $E_x$ has the property that local consistency with locality $\ell$ implies global correctness. (2) For every gate $g$ in $E_x$ the sub-circuit of $E_x$ computing $g$ is of size at most~$\gamma$.

The length of the $\SNARG$ is $\poly(\secp,\ell,\log{|E_x|})$, the length of the $\crs$ is $\gamma\cdot \poly(\secp)$,\footnote{One could strengthen this result to make the $\crs$ grow only with the (possibly succinct) description of the circuit computing each gate~$g$.  For the sake of simplicity we chose to avoid this extra layer of complication in the technical section.}   and non-adaptive soundness holds assuming the $|E_x|$-hardness of $\LWE$.
\end{theorem}

We deduce \cref{thm:main-intro} by combining \cref{thm:intro:ext-super-poly} with a construction of such locally unsatisfiable extensions for any $\mathsf{NP}$ language $\mathcal L$ with bounded space propositional proofs of unsatisfiability (see the full version for details).

\znote{Should we mention here about the potential towards NP? So that the readers would be more interested} \vnote{Do you mean your observation that a $\sqrt{|w|}$-size proof, and therefore a fully succinct proof via bootstrapping, *may* be possible for all of NP?} \ynote{Let's talk about this.  Not sure what to say here given that we may have too large blowups.}

\subsection{Related Work}\label{sec:related}
%\ynote{in progress...}\vnote{I gave it a shot, feel free to edit/rewrite}

There is a large body of work, especially in recent years, that construct $\SNARG$s under standard hardness assumptions for more and more expressive languages                                          
                                                                                                     
                                                                                          %Indeed, much of the work is on constructing non-signaling $\PCP$s \cite{?,?}. 
In what follows, we restrict ourselves to discussing the most closely related works, the ones that break the non-signaling barrier, and construct $\SNARG$s for languages that we believe do not have non-signaling $\PCP$s. Similarly to our work, all these works provide non-adaptive soundness.

%\paragraph{Comparison with \cite{STOC:SahWat14}.} 
%Sahai and Waters~\cite{STOC:SahWat14} constructed the first SNARG system for all of NP, without relying on random oracles or knowledge assumptions. Their SNARG system had proofs of length $O(\secp)$, independent of the statement or witness length, and a common reference string of length $O(w)$, where $w$ is the length of the NP witness. In contrast to \cite{STOC:SahWat14}, our SNARG system supports a subclass of NP, and our proof size grows logarithmically with the length of the (propositional) coNP witness, or at least the space required to verify it. On the other hand, while \cite{STOC:SahWat14} required the full power of indistinguishability obfuscation, 
%\ynote{I think they rely on poly-time iO, but when converting this to a falsifiable assumption it becomes $2^{|x|}$ assumption}  our constructions are based on a single, simple falsifiable assumption, namely the polynomial hardness of the learning with errors problem. Our construction permits a transparent setup, meaning that our CRS is truly random. \vnote{check!} Finally, our construction admits a potentially smaller CRS, of size proportional to the space required to verify a co-non-deterministic proof for the language in question which, in general, is shorter than the witness length, perhaps even exponentially so.

%\ynote{The next paragraph is a slight rewording:}

\paragraph{Comparison with \cite{STOC:SahWat14}.} 
Sahai and Waters~\cite{STOC:SahWat14} constructed the first $\SNARG$ system for all of $\NP$, without relying on random oracles or knowledge assumptions. Their $\SNARG$ system has proofs of length $O(\secp)$, independent of the statement or witness length, and a $\CRS$ of length $O(|w|)$, where $|w|$ is the length of the $\NP$ witness. In contrast to \cite{STOC:SahWat14}, in our $\SNARG$ system the proof size also grows poly-logarithmically with the length of the propositional proof of unsatisfiability. On the other hand, our $\CRS$ has length proportional to the space required to verify the propositional proof, which in general is shorter than the witness length, perhaps even exponentially so.

Importantly, \cite{STOC:SahWat14} requires the full power of secure indistinguishability obfuscation, which when converted into a falsifiable assumption, becomes a $2^{|x|}$-hardness assumption (where $x$ is the instance).%In addition their assumption is not post-quantum secure. 
~In contrast, our constructions are based on a single, simple, falsifiable, post-quantum assumption, namely the $\poly(T)$-hardness of $\LWE$, where $T$ is the length of the propositional proof.

Finally, our construction permits a transparent setup, meaning that our $\CRS$ can be generated using public coins, whereas the $\CRS$ in the \cite{STOC:SahWat14} construction consists of an obfuscated circuit. %\znote{Do we need to mention the post-quantum security aspect?} \ynote{good point, added!}

%+ better assumption \\ 
%+ potentially smaller CRS (for any given language) \\ 
%+ transparent setup \\
%- only supports a subclass of NP \\ 
%- proof size grows (vs. constant in SW)

\paragraph{Comparison with \cite{FOCS:JaiJin22}.} Our work is inspired by the work of Jain and Jin~\cite{FOCS:JaiJin22}, which pioneered the idea of using co-non-deterministic proofs for a language $\cL$ to improve the assumption in \cite{STOC:SahWat14} from a $2^{|x|}$-hardness assumption to an assumption falsifiable in time \emph{less than} $2^{|x|}$. Specifically, in \cite{FOCS:JaiJin22}, they are able to rely on the $2^{|x|^\epsilon}$-hardness of falsifiable assumptions (used to build indistinguishability obfuscation for circuits of input length $|x|^\epsilon$) to instantiate a new variant of the \cite{STOC:SahWat14} $\SNARG$. 

We improve on \cite{FOCS:JaiJin22} in several ways: they construct a $\SNARG$ for all $\NP$ languages $\cL$  that have polynomial-size propositional proofs for $x\notin \cL$, and their soundness relies on indistinguishability obfuscation for circuits with security parameter input length. 
We construct a $\SNARG$ for the same $\NP$ languages assuming the polynomial hardness of $\LWE$. In addition, \cite{FOCS:JaiJin22} inherits the trusted setup of \cite{STOC:SahWat14} while our scheme has transparent setup.  Finally, we construct $\SNARG$s for a richer class of languages: as described in \cref{thm:main-intro}, our construction can work with a propositional proof for non-membership which may be of super-polynomial size~$T$, as long as it can be verified in polynomial space.  %Our $\CRS$ grows with the space required to verify the propositional proof, our $\SNARG$ grows with  $\poly(\log T)$  and our assumption is the $\poly(T)$-hardness of $\LWE$.

%+ better assumption \\ 
%+ smaller CRS (grows with space not length of prop proof)  \\
%+ transparent setup \\

%\alex{We need to discuss \cite{FOCS:JaiJin22}, which already handles poly-size proofs assuming sub-exp FE/iO.}

\paragraph{Comparison with \cite{C:BBKLP23}.}  Our work also draws inspiration from \cite{C:BBKLP23}, which  constructs a $\SNARG$ with non-adaptive soundness from the polynomial hardness of $\LWE$ for any monotone batch $\NP$ language.  
Their construction relies on the hash-and-$\BARG$ blueprint, but they use a special hash family, which they call {\em predicate extractable}. Looking into the details of this predicate-extractable hash function, one can think of it as a \emph{commitment} to, and \emph{quasi-argument} about, the output of an encrypted, instance-dependent extended circuit. Indeed, there is a specific, simple locally unsatisfiable extension implicit in \cite{C:BBKLP23}, and as a result our main theorem implies the result of \cite{C:BBKLP23} as a corollary (albeit with a slightly different construction and analysis).

Importantly, such languages are not known to have non-signaling $\PCP$s, and thus \cite{C:BBKLP23} was the first to break the ``non-signaling $\PCP$ barrier". However, the monotone policy batch languages considered in \cite{C:BBKLP23} were still \emph{easy} in that they could be decided in time $2^{\ell}$, where $\ell$ denotes the SNARG proof length. In contrast, in this work we construct SNARGs for \emph{hard} languages such as $\mathsf{DDH}$, which is a much more powerful result. 


\ifnum\cameraready=0
\paragraph{Roadmap.} We first present our general method for constructing $\SNARG$s. 
 Specifically, \Cref{thm:intro:ext-poly} is formalized and proved in \Cref{sec:extended-circuit-snarg}, and 
\Cref{thm:intro:ext-super-poly} is formalized and proved in  \Cref{sec:super-poly-extension}. Then we focus on propositional proofs.  \Cref{thm:main-intro} is formalized and proved in \Cref{sec:proof-to-extended-circuit,sec:super-poly-EF} and in \Cref{sec:ext-ckt-app} we derive the corollary for $\DDH$ (\Cref{cor:DDH}).  %\ynote{Add graph isomorphism}
\fi 




\section{Technical Overview}\label{sec:techniques}

Our starting point is the blueprint of constructing a $\SNARG$ via the hash-and-$\BARG$ paradigm \cite{FOCS:ChoJaiJin21,TCC:KalVaiZha21}.  In this construction, to prove that $x\in\cL$, the prover first uses its witness to compute a ``transcript'' $\tau$ containing the values of all the wires of the verification circuit $C_x$. Then, the prover hashes $\tau$ using a somewhere extractable hash function with local opening~\cite{ITCS:HubWic15}, to obtain a hash value~$\hval$.  Such a hash function is associated with a hash key and a trapdoor.  The hash key is used to generate the hash value~$\hval$, and the trapdoor can be used to extract a few input values from~$\hval$. In what follows, we denote the number of locations that can be extracted by~$\ell$, and note that the hash values and the hash key grow linearly with~$\ell$.  The prover also adds a proof that these hashed wire values satisfy all the gates of the circuit, by using a non-interactive batch argument ($\BARG$)\cite{FOCS:ChoJaiJin21}.  Namely, the prover appends to the hash value~$\hval$ a $\BARG$ that proves that for every gate $g$ of $C_x$ there is an opening to the input and output wires of~$g$ such that these openings are valid w.r.t.~$\hval$ and they respect the gate. Alternatively (which is the approach taken in this paper), one can commit to $\tau$ using an ordinary hash tree, provided that the $\BARG$ satisfies a notion called ``somewhere extractability.'' 

It is well known that one can efficiently convert any cheating prover for this hash-and-$\BARG$ construction into a {\em local assignment generator}, denoted by $\localgen$, which is a randomized algorithm that takes as input $\ell$ wires (where $\ell$ is the number of wires that can be extracted from the hash value~$\hval$), and outputs an assignment to these wires, with the following guarantees:
\begin{enumerate}
    \item {\bf Local consistency:} The assignment is locally consistent (i.e., it respects all the gates).
    \item  {\bf Non-Signaling:} for any two possible wire sets $T_0,T_1$ of size at most $\ell$, the distribution of the assignments for the wires in $T_0\cap T_1$ in $\localgen(T_0)$ and in $\localgen(T_1)$ are computationally indistinguishable.
\end{enumerate}


Unfortunately, it is well known that such local consistency guarantee does not always imply global correctness. Indeed, starting from the work of \cite{STOC:KalRazRot14}, there have been several attempts to {\em extend} the verification circuit~$C_x$ into an extended version, which we denote by $E(C_x)$, such that local consistency of the extended circuit $E(C_x)$ does imply global correctness. Unfortunately, these attempts have limitations.  It is known that such an extension exists only for languages that have a $\PCP$ with non-signaling soundness, which in turn is known to limit the $\SNARG$ to be of size at least $\ell$ for $\NP$ languages that require time $2^\ell$ to decide. 

\iffalse 

\paragraph{New Insight}  Our new insight is that in the non-adaptive setting, this extension can depend on the instance $x$, in an {\em inefficient} way.  Namely, suppose for any fixed $x\notin \cL$ there is a way to extend the verification circuit $C_x$ into a new verification circuit $E_x$\footnote{Namely,  $E_x$ is obtained by adding wires and gates to $C_x$} such that local consistency of $E_x$ implies that the specific wire of $E_x$ corresponding to the output wire of $C_x$ must be~$0$.   In this case we can ask the cheating prover to hash-and-$\BARG$ the extended circuit $E_x$ and thus obtain soundness.

\fi 

\paragraph{New Insight.}  Our new idea is to consider \emph{inefficient}, \emph{instance-dependent encodings} of the circuit $C_x$. Namely, suppose for any fixed $x\notin \cL$ there is a way to extend the verification circuit $C_x$ into a new verification circuit $E_x$\footnote{Namely,  $E_x$ is obtained by adding wires and gates to $C_x$} such that local consistency of $E_x$ implies that the specific wire of $E_x$ corresponding to the output wire of $C_x$ must be~$0$. We call such a family $\{E_x\}$ a locally unsatisfiable extension of the circuit $C$. 

A naive proposal would be to ask the prover to hash-and-$\BARG$ the extended circuit $E_x$ and thus derive soundness from the local unsatisfiability of $E_x$. Unfortunately, it seems like we are in a lose-lose situation:

\begin{itemize}
    \item If $E_x$ can be computed efficiently from $C_x$, then we can essentially think of the extension as being independent of~$x$, by thinking of the new extended circuit as being $E(C_x)$, similar to prior works. 
    \item On the other hand, if $E_x$ \emph{cannot} be computed efficiently from $C_x$, then the prover does not know what computation to run, so we do not have completeness. 
\end{itemize}
%Moreover, even if we somehow manage to get around this lose-lose situation, we will still be limited to extensions such that the size of $E_x$ is at most polynomial in the size of $C_x$, since otherwise the (honest) prover will run in super-polynomial time. This limits us to languages in $\NP\cap\coNP$.
Additionally, even if the prover magically knew a description of the circuit $E_x$, if $E_x$ has super-polynomial size the honest prover cannot even evaluate it. 

Nevertheless, we give a construction of a $\SNARG$ assuming the \emph{existence} of a locally unsatisfiable extension $\{E_x\}$ of the $\mathsf{NP}$ verification circuit $C$, despite being unable to compute what it is. Our construction can handle \emph{any} polynomial-size such extension, and moreover can handle extensions where the size of $E_x$ is super-polynomial, as long as each individual wire value of $E_x(w)$ is efficiently computable from the input.  

\paragraph{The encrypt-hash-and-$\BARG$ paradigm.} How do we construct a $\SNARG$ that makes use of the existence of $E_x$ without being able to compute it? We ask the prover to give a hash-and-BARG for a \textbf{hidden, encrypted computation} that is not checked in the clear. Namely, we include in the $\crs$ a ciphertext (using fully homomorphic encryption), which in the actual scheme can be an encryption of the all-zero string, but in the analysis we will think of this ciphertext as encrypting the description of the extension $E_x$. The $\SNARG$ is publicly verifiable, and hence the success probability of a cheating prover does not change when the encryption of the zero string is replaced with an encryption of the description of $E_x$. 

In our construction, the prover hash-and-$\BARG$s the original circuit~$C_x$ and additionally computes the values of all the wires of the (homomorphically evaluated) encrypted extended computation, and adds a hash-and-$\BARG$ for this encrypted computation. More specifically, we think of the extended circuit $E_x$ as first computing $C_x$ and then computing a circuit $D_x$ that takes as input all the wires of $C_x$.  The prover, in addition to hashing all the wires of $C_x$ and computing the corresponding $\BARG$, will consider the encrypted computation $\Eval(U_{D_x},\cdot)$, that takes as input all the wires of $C_x$ and a description $\langle D_x \rangle$ of a circuit, and evaluates the circuit $D_x$ on these wires ``under the hood'' of the encryption. The prover will hash-and-$\BARG$ this encrypted computation, except for the input which is already hashed. The verifier simply verifies the two hash-and-$\BARG$s.

Note that even though in the actual scheme the prover never gives any useful information about $E_x$, in the analysis we replace the all zero encryption with the encryption of 
an encryption of $\langle E_x\rangle$ (or $\langle D_x\rangle$). The punch line of this approach is that we can show that given a cheating prover for this ``encrypted-hash-and-BARG'' on a non-adaptively chosen input $x$, one can obtain a local assignment generator for the circuit $E_x$. This requires handling two technical issues:

\begin{itemize}
    \item The computation of $E_x$ is \emph{encrypted} rather than in the clear. Essentially, one needs to show that a local assignment generator for the encrypted computation implies a local assignment generator for the computation ``underneath'' the encryption. This is proven assuming that the FHE scheme has gate-by-gate evaluation and satisfies a standard notion of malicious correctness.
    \item Even ``underneath the encryption,'' what is evaluated is a \emph{universal circuit} $U$ on input $(\langle E_x \rangle, w)$ rather than the circuit $E_x$ on $w$. Thus, one needs to show that local assignment generators are roughly preserved under the universal circuit transformation.
\end{itemize}

We handle these technical issues and show that a local assignment generator for $E_x$ can still be constructed. Thus, soundness holds assuming a local assignment generator for $E_x$ implies global correctness. We refer the reader to the full version for further details.



\paragraph{Handling extensions of super-polynomial size.}
In the encrypt-hash-and-$\BARG$ paradigm described above the $\crs$ includes an encryption of the description of the extended circuit.  Thus, if the description is of super-polynomial size the $\crs$ is of super-polynomial size. 
We show how to extend this paradigm and show how to construct $\SNARG$s even for languages that have locally unsatisfiable extensions of {\em super-polynomial} size, as long as each gate in the extension can be computed in polynomial time. 

The basic idea is the following:  rather than having the prover hash-and-$\BARG$ the entire (encrypted) extended  computation, we will ask the prover to hash-and-$\BARG$ only parts of this (encrypted) computation.  More specifically, the $\crs$ will include an encryption of only the computation of $\ell$ gates of the $\ell$-locally unsatisfiable extension. We will assume that computing only $\ell$ gates can be done in polynomial time.
This suffices since to compute the underlying $(\ell,\epsilon)$-local assignment generator we only need the prover to compute $\ell$ gates of the underling computation. 

Unfortunately, this idea does not quite work due to a ``signaling'' issue. In particular, an adversary, who is given a description of the circuit computing the relevant $\ell$ gates $g_1,\ldots,g_\ell$, under the hood of an $\FHE$,  may provide wire values (under the hood of the $\FHE$) that may depend on all these $\ell$ specific gates, and thus break the non-signaling requirement of the underlying $(\ell,\epsilon)$-local assignment generator.
%(as defined in \Cref{def:local-assignment-gen}).
At first, it may seem that this is not a concern since any (cheating) prover commits to all the wires in the circuit $C_x$ ``in the clear'' (i.e., not under the hood of the $\FHE$). Recall that these wires are the input to the extended circuit, and hence once these wires are committed to, it seems like the provers' hands are tied, and thus it cannot signal.  This intuition indeed holds for $\log$ depth extensions.  However, for deep extensions, this is no longer the case due to an ``exponential error growth.''  %Namely, the local consistency is associated with a probability of error 


It is tempting to try to address this signaling problem by encrypting each of these $\ell$ computations with a different (independent) key.  However, this solution brings rise to a new issue, which is that of consistency.  The issue is that these $\ell$ computations may share some wires, and it is not clear how to enforce that the value of these shared wires are consistent.

Instead, we solve the signaling issue by adding to the $\crs$ $\ell$ ciphertexts, where the $i$'th ciphertext encrypts the  computation $g_i$ and is encrypted with a fresh public key~$\pk_i$. The hope is to argue in the analysis that the value of the gate $g_i$ encrypted under the key $\pk_i$ is the same as the value of this gate when encrypted under public key~$\pk$ used for encrypting the joint computation $g_1,\ldots,g_\ell$, thus establishing the non-signaling requirement.  To argue that such consistency condition indeed holds is tricky due to the exponential blowup in error. We overcome this exponential blowup using the idea of circuit extension, originating from \cite{STOC:KalRazRot14}. Specifically, the prover will extend the computation of each $g_i$ to include the low-degree extension of each layer of the computation.  Then one can argue by induction on~$j$, that the value of each gate in layer $j$ of the two computations of $g_i$ are identical.  We refer the reader to the full version for further details.


% -------------
% We observe however, that we use the prover only to read a few wires in this extended circuit. Indeed, it suffices to encrypt only the description of $\ell$ sub-circuits, each computing a single gate.  This observation allows us to deal with super-polynomial extensions as long as each gate in the extension can be computed in polynomial time (or more generally, has a polynomial size description). 



%\paragraph{Comparison with \cite{C:BBKLP23}.}  Our work draws inspiration from \cite{C:BBKLP23}, which  constructs a $\SNARG$ under $\LWE$ for any monotone batch $\NP$ language.  Importantly, such languages are not known to have non-signaling $\PCP$s, and thus this work was the first to break the ``non-signaling $\PCP$ barrier". Their construction relies on the hash-and-$\BARG$ blueprint, but they used a special hash family, which they call {\em predicate extractable}.  One can think of this predicate extractable hash as a specific instance-dependent extension, and hence we view our work as an extension and generalization of their work. 

% Specifically, a monotone batch $\NP$ language is associated with an $\NP$ language $\cL$ and a monotone circuit $\cM$.  an instance $(x_1,\ldots,x_k)$ is in the monotone batch $\NP$ language, denoted by $\cL_\cM$ if and only if it satisfies $$\cM(1_{x_1\in\cL},\ldots,1_{x_k\in\cL})=1$$
% The reason why the hash-and-$\BARG$ paradigm is not known to imply soundness is due to the exponential error blowup. 

\paragraph{Applications and Connections to Propositional Proofs}

Armed with the new paradigm for constructing $\SNARG$s we now ask: {\em which $\NP$ languages have instance specific extensions for which each gate can be computed in polynomial time and for which local consistency implies global correctness?}

We emphasize that this is a particularly challenging question, since it is unclear how to prove that local consistency implies global correctness. To prove such a statement, the mathematical proof we write needs to crucially rely on the fact that $C_x$ is not satisfiable. Otherwise, the same mathematical proof would go through if $C_x$ is indeed satisfiable.% which indicates that the proof is wrong. Indeed, the construction of SNARGs for NP from iO \cite{STOC:SahWat14} implicitly enumerates all possible NP witnesses. This is why an exponential length mathematical proof $\pi_x$ exists for every $x \notin L$ in their construction, where $\pi_x$ proves that their reduction $R_x$ is indeed a correct reduction.

As we mentioned earlier, in this work, we seek to understand if we can build $\SNARG$s for languages in $\NP \cap \coNTIME(T)$, with a reduction that runs in time $\poly(T)$. As an initial attempt, let's consider a general language $\lang$ in $\NP \cap \coNTIME(T)$ with $\NP$ verifier $M$ and $\coNTIME$ machine $\bar{M}$. If we try to build $\SNARG$s for this general $\lang$ (and hence general $M$ and $\bar{M}$), we will encounter a similar issue as before. The issue is that, unless our mathematical proof of ``local implies global'' property crucially uses the fact that $M$ and $\bar{M}$ are indeed the verification machines of $\lang$ and $\bar{\lang}$, respectively, there is no hope to write down a correct proof. 

In summary, it seems that the issue is that the non-deterministic witness for $\bar{\lang}$ \emph{lacks structure}. More precisely, without knowing more structure about the mathematical statement ``$\forall w, C_x(w) = 0$'' or ``$\bar{M}$ indeed decides $\bar{\lang}$'', the best we can do in the reduction is to treat $C_x$ as a black-box, and enumerate all possible witness $w$ to check that the mathematical statement indeed holds. However, this means the reduction needs to run in $2^{|w|}$ time, in which case we cannot hope to achieve succinctness in our $\SNARG$ construction.

\znote{I feel the discussion is necessary, otherwise the reader will ask why prop proofs (e.g. Vinod :) ).}

To overcome this barrier, we draw the inspiration from the recent work \cite{FOCS:JaiJin22}, which shows that, assuming a little more structure of the non-determinsitic witness of $\bar{\lang}$, they can avoid the $2^{|w|}$-reduction using iO. The additional structure they impose on the non-determinsitic witness of $\bar{\lang}$ is that the witness is a \emph{propositional logic} proof.
In this work, we show that if there exists a propositional logic proof of unsatisfiability, then we can build the extended circuits. 

\paragraph{Background of Logic.} We recall propositional logic systems with extension rules (i.e. Extended Frege systems) \cite{krajicek95}. Such a logic system is defined as a tuple of variables and connectives such as ``$\land$'', ``$\lor$'', ``$\impl$'', ``$\neg$'', ``$\logicequiv$'', which represent ``and'', ``or'', ``imply'', ``negation'', and ``equivalent'', respectively. 
A proof in such a logic system is a sequence of ``lines'', where each line is a formula derived via one of the following rules.
\begin{itemize}
    \item {\bf Axioms.} The formula is a constant size tautology, which means for every truthful assignment, the formula is evaluated to $1$.
    
    \item {\bf Modus Ponens.} There exist two formulas $f, g$ such that the formulas $f, g, f \impl g$ are the lines somewhere before the current line, and the current line is the formula $g$.
    
    \item {\bf Extension Rule.} The line is in the form $v \logicequiv \phi$, where $v$ is a variable that has not appeared before the current line, and also does not appear in $\phi$. 
\end{itemize}
The size of a formula is the length of the binary string that is used to write down such a formula, including all the punctuations. The size of a proof is the total size of the lines in the proof.

The extension rule can be used to shorten the size of each line in the proof, by introducing new propositional variables to the subformulas used in the proof. Indeed, one can assume without loss of generality that each line of the proofs in the Extended Frege system is a constant size formula, without significantly blowing up the size of the proofs.



We first describe how to build a polynomial-size extended circuit, if the propositional logic proof is polynomial size. Indeed, our construction of the extension circuit for polynomial-size propositional proofs is almost identical to the padded circuit used in \cite{FOCS:JaiJin22}. We describe the construction again in the context of the extended circuits.

\paragraph{Extension from Polynomial Size Propositional Proofs.} The key \emph{structural property} of propositional logic proofs is that each line of the proof is a formula, and hence is naturally a circuit. Hence, we can use them in our construction of $E_x$. Moreover, the proof is \emph{local}, which means that the truthfulness only depends on a constant number of previous lines. Recall that, we assume without loss of generality that each line of the proof has a constant size. 

Bearing these structural properties in mind, given a propositional logic proof $\theta_1, \ldots, \theta_T$ for the unsatisfiability of $C_x$, the initial attempt to build $E_x$ is as follows. For each $\theta_i$, we build a circuit $C_i$ that computes $\theta_i$, and add $C_i$ in $E_x$. To prove the local-to-global property, our intuition is that, since each line must be true, the circuits $C_i$'s must output $1$'s. Moreover, we hope to use an inductive argument to show that this is indeed true if we extract the output of $C_i$ using the local assignment generator. For example, suppose $\theta_i$ is derived from $\theta_{i_1}, \theta_{i_2}, \ldots, \theta_{i_c}$, then we can extract the outputs of $C_{i_1}, \ldots, C_{i_c}, C_i$ to argue that, if all the circuits $C_{i_1}, \ldots, C_{i_c}$ outputs $1$, then $C_{i}$ must also output $1$. Finally, the last circuit $C_{T}$ must compute a function checking whether $\out$ is $0$ or not, where $\out$ is the output gate of $C_x$. This is because a propositional proof must end with the statement, and in our case, the statement is ``$\out = 0$''. Hence, if we can use the aforementioned inductive argument to show that $C_T$ outputs $1$, then it implies $\out = 0$. In this way, we can argue that local consistency implies global correctness.

However, the above initial attempt does not work directly, because a closer examination will reveal that the security loss in such an inductive argument is exponential in the length of the proof. The reason is that, for each $\theta_i$ that follows from an inference rule, the indices $i_1, \ldots, i_c$ may be different for each $i$, and they may not follow any pattern. Recall that in the inductive argument above, before arguing that $C_i$ must output $1$, we need to extract $C_{i_1}, \ldots, C_{i_c}$ and prove that they all output $1$ first. However, when we transit from the index $(i-1)$ to $i$ in the inductive argument, it is possible that the outputs of $C_{i_1}, \ldots, C_{i_c}$ have not been extracted. A potential solution to this issue is to extract all the outputs of $C_1, \ldots, C_{i-1}$, but we cannot afford such locality in the local assignment generator.

To resolve this issue, we need to have a mechanism that allows us to ``succinctly'' memorize the fact that we have proven that the outputs of $C_1, \ldots, C_{i-1}$ are all $1$'s, by only extracting a small number of wires and gates in $E_x$. We achieve this by building a binary tree of $\sfAND$ gates, where the leaf nodes of the tree are the outputs of $C_1, \ldots, C_T$. In the inductive argument, at the $i$-th step, we extract $O(\log T)$ roots of some sub-trees in the binary tree. Those roots are chosen such that the leaves of those roots consist of the first $i$ leave nodes. Now to ensure the first $i$ circuits output $1$, we only need to examine whether those roots output $1$ or not. For more details, see the full version.

\medskip
So far, we have only shown how to handle polynomial-size propositional logic proofs. If the propositional logic proof is of super-polynomial size, the number of leaves in the $\sfAND$ tree is super-polynomial. Then it is not clear how to compute the root node of the $\sfAND$ in polynomial time, since the root of the tree depends on the values of all the leaves.

\paragraph{Towards Super-polynomial Size Propositional Proofs.}
To extend the idea to super-polynomial size propositional proofs, our key observation is that, the procedure of adding $C_i$'s to the leaves of the $\sfAND$ tree is similar to writing down a mathematical proof on a piece of paper, where the space of the paper is limited. Note that, sometimes we can erase some formulas on the paper and rewrite new formulas there, as long as the formulas can be derived only using the remaining formulas on the paper. Then we can reuse the space of the paper and write long proofs. This motivates us to define a space notion of propositional proofs, and only keep the formulas in the space on the leaves of the $\sfAND$ tree. 

Indeed, space complexity has been defined for propositional logic proofs \cite{InfoComp:EstJac01,SIAM:ABRW02}. However, to the best of our knowledge, those definitions only define space complexity for propositional proof systems without the extension rule. However, in our setting, we can handle the extension rule by adding new gates in $E_x$. Specifically, we can have each extended variable be associated to a new gate in $E_x$, and use the defining formula of the variable to specify how the gate should be computed from existing gates. 

\paragraph{Defining Space of Extended Frege Proofs.} In this work, we introduce a new definition of the space complexity for propositional proofs with extension rules (i.e., for extended Frege systems). In our definition, at any point in the derivation of the proof, we maintain a set of formulas as the ``memory'', and we require that new formulas (resp. new variables) must be derived from existing formulas (resp. variables) in the memory. We also allow the erasure of the formulas in the memory. However, if the erased formula is the defining formula of some variable $v$, then we further require that the variable is not used later in the proof. The space complexity of the proof is then defined as the maximum total size of the formulas in the memory throughout the derivation of the propositional proof.
For more details, see the full version.

We will show that if a circuit $C_x$ has propositional proofs of unsatisfiability, where the proof has polynomial space, then we can build an extended circuit $E_x$, where the size of the circuit grows with the size of the propositional proof, which we allow it to be super-polynomial. However, each gate in the extended circuit can be computed using a polynomial-size subcircuit. From our aforementioned construction of SNARGs via Encrypt-Hash-and-BARGs, this would give us SNARGs with CRS size growing with the space of the propositional proof, and SNARG size grows only \emph{logarithmically} in the size of the propositional proofs. 

\paragraph{Extended Circuits from Bounded-Space Proofs.}
The construction of the circuit extension $E_x$ is as follows. Our starting point is our aforementioned $\sfAND$ tree construction in the case of polynomial-size propositional proofs. To ensure the $\sfAND$ tree is polynomial size, our idea is to build the $\sfAND$ with only $s$ leaves, where $s$ is a polynomial upper bound on the space. However, it remains to handle the erasure operation in propositional proofs.
A natural idea is to build a ``dynamic'' $\sfAND$ binary tree, with insertions and deletions of the leaves. However, it is not clear if we can delete the gates in $E_x$ during the construction procedure of $E_x$. Because if we delete the gates, what is the point of adding them in the first place?

\begin{figure}[h!]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\begin{tikzpicture}[
  level distance=1.5cm,
  level 1/.style={sibling distance=3cm},
  level 2/.style={sibling distance=1.5cm}
]
  \node {$\land$}
    child {
      node {$\land$}
      child {node {$1$}}
      child {node {$2$}}
    }
    child {
      node {$\land$}
      child {node {$3$}}
      child {node {$4$}}
    };
\end{tikzpicture}
%\caption{Original $\Delta_s^0$ circuit.}
\end{minipage}
%\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\begin{tikzpicture}[
  level distance=1.5cm,
  level 1/.style={sibling distance=3cm},
  level 2/.style={sibling distance=1.5cm},
  circled/.style={rectangle, draw, inner sep=2pt, circle, minimum size=10pt}
]
  \node (R) {$\land$}
    child {
      node (L) {$\land$}
      child {node (A) {$1$}}
      child {node (B) {$2$}}
    }
    child {
      node (RC) {$\land$}
      child {node (C) {$3$}}
      child {node (D) {$4$}}
    };
  \node [right=0.15cm of L] (X) [circled] {$\land$};
  \node [right=0.15cm of B] (B') [circled] {$2'$};
  \node [right=0.6cm of R] (R') [circled] {$\land$};
  \draw (X) -- (A);
  \draw (X) -- (B');
  \draw (R') -- (X);
  \draw (R') -- (RC);
\end{tikzpicture}
%\caption{$\Delta_s^0$ and $\Delta_s^1$, after erase the formula assigned to the $2$-th leaf node.}
\end{minipage}
\caption{An example of inserting a new leaf-to-root path for the second leaf node. Left: original $\sfAND$ tree circuit. Right: circuit after adding a new leaf-to-root path for the second leaf node. The new gates are marked in circles.}
\label{fig:intro-erase-formula}
\end{figure}

To deal with deletions, our idea is to use insertions to ``emulate'' deletions, as follows. To delete a leaf node, instead of really deleting it, we build an entire new root-to-leaf path for that leaf node \emph{on top of the original tree}. Namely, the children of the gates on the new root-to-leaf path are set to be the nodes in the original tree, if the child is not included in the root-to-leaf path. We show an illustrative example in \Cref{fig:intro-erase-formula}.
Then we set the new leaf node on the new root-to-leaf path as a constant $1$. Now if we only look at the sub-circuit that the new root in the root-to-leaf path depends on, it is still a binary tree, but now the second leaf can be regarded as ``deleted'', because its value is set to be a constant $1$, which does not affect the output of the $\sfAND$ tree.

In summary, to build $E_x$, we start with a binary tree of $s$ leaves, where $s$ is the space of the propositional proof. Initially, all the leaf nodes are set to output the constant $1$. Then we iterate through the lines in the proof. If the new line is derived via an inference rule, then we add a subcircuit $C_i$ computing the truth value of that line. Then we choose a leaf node that has not been assigned before. We create a new root-to-leaf path as above for that leaf node, and assign the output of $C_i$ to the new leaf node. For the erasures, we find the leaf node that was assigned to the sub-circuit computing the formula being erased, and create an entirely new root-to-leaf path to it, and set the new leaf node to be the constant $1$. Finally, we take the resulting circuit as $E_x$. 

The proof that local consistency implies global correctness follows from the same high-level idea as the polynomial-size propositional proof case, but there are more technical issues in the detail. For example, we need a new mechanism to succinctly memorize that all the inputs to the $\sfAND$ tree are all $1$'s, because now the order of assigning $C_i$'s to the leaves is no longer monotonous and consecutive, since the position of the newly assigned leaf may be arbitrary among all the leaves.
For more details, see the full version.

\paragraph{On the Provability of Propositional Logic.} So far, we have shown how to build SNARGs from LWE, if the language has a polynomial-size or bounded-space proportional proof of non-membership. It remains to ask, \emph{for what languages do we have a propositional proof of non-membership?} More broadly, one may ask \emph{what mathematical theorems can be formalized in polynomial-size or bounded-space propositional logic proofs?}

Indeed, the latter question is one of the central questions in \emph{proof complexity}. On the positive side, the \emph{bounded arithmetic} developed by Cook \cite{STOC:Cook75}, Buss \cite{Buss86}, and many others shows that if a proof can be formalized in certain sub-theories of Peano arithmetic, then the proof can be translated to propositional proofs of certain lengths in Extended Frege systems. Moreover, any language in $\NP$ has a propositional proof of non-membership of size exponential in the length of the NP witness. However, it is unlikely that such a proof can always be polynomial size. Indeed, it has been shown \cite{JSL:CooRec79} that if every tautology has a polynomial-size propositional proof, then $\NP = \coNP$.

In this work, we rely on the propositional translation \cite{STOC:Cook75, Buss86} to show that the Diffie-Hellman language (DDH) has a polynomial-size propositional proof of non-membership. As an application, we show how to build SNARGs for DDH.

\paragraph{Applications to Diffie-Hellman Language.} Recall that the Diffie-Hellman language is defined as
$$\lang = \family{(g, h, g^w, h^w) \mid g, h \in \bbG, w \in \mathbb{Z}_q},$$
where $\bbG = \{\mathbb G_n\}_n$ is an asymptotic family of cyclic groups of order $q = O(2^n)$. Let $x = (g, h, g', h')$ be a fixed instance with $x \notin \lang$, we want to show that the verification circuit $C_x(w)$ for $\lang$ has polynomial-size propositional proof of unsatisfiability. Note that for any such fixed $x$, there exists a fixed $s \in \mathbb{Z}_q$ such that $h = g^s$ and $h' \neq {g'}^s$. Then we can write down a mathematical proof that $C_x$ is not satisfiable, as follows.
\begin{itemize}
    \item Suppose $C_x(w) = 1$ for some $w$, then $g' = g^w$ and $h' = h^w$.
    \item From $h = g^s$, this means that $h' = h^w = (g^s)^w$. 
    \item $(g^s)^w = (g^{w})^s = {g'}^s$. We reach a constriction with $h' \neq {g'}^s$. Hence, $C_x(w)$ is unsatisfiable.
\end{itemize}
We observe that each step of the above mathematical proof can be converted to polynomial-size propositional proof using Cook's propositional translation \cite{STOC:Cook75}. Putting them together, we obtain a polynomial-size propositional proof of unsatisfiability of $C_x$.
For more details, see the full version of this paper.

%We first observe that every $\NP$ language has such an extension of size exponential in the witness length:  The extension simply computes $C_x(w)$ for every possible $w$.


%\input{Notes2Self}

==> App-GI.tex <==
\subsection{SNARGs for Graph Isomorphism Language}
In this section, we show how to build SNARGs for the graph isomorphism language for strongly regular graphs. We first recall the definition of strongly regular graphs. 

\begin{definition}[Strongly Regular Graph]
    A \vnote{undirected?} graph $G = (V, E)$ is said to be $(v, k, \lambda, \mu)$-strongly regular, if $|V| = v$, each vertex has degree $k$, and
    \begin{itemize}
        \item For any two vertices $x, y$ with $(x, y) \in E$, $|\neighbor(x) \cap \neighbor(y)| = \lambda$.
        \item For any two vertices $x, y$ with $(x, y) \notin E$, $|\neighbor(x) \cap \neighbor(y)| = \mu.$  
    \end{itemize}
    where $\neighbor(x)$ is the neighbor set of $x$, for any $x \in V$.
\end{definition}

We prove the following theorem.

\begin{theorem}[SNARGs for Graph Isomorphism Language]\label{thm:SNARGs-Graph-ISO}
Assuming $2^{\secpar^{0.9}}$-security of LWE, there exists a SNARG for the following promise language $\langISO = (\lang_\YES, \lang_\NO)$,
\begin{align*}
    \lang_\YES = \left\{(G_1, G_2) \middle| 
    \begin{aligned}
     G_1, G_2 \text{ are strongly regular graphs, } \\ \exists \text{ isomorphism } \phi: G_1 \rightarrow G_2.
    \end{aligned}
     \right\},
\end{align*}
 \begin{align*}
\lang_\NO = \family{(G_1, G_2) \mid G_1, G_2 \text{ are non-isomorphic strongly regular graphs}},
\end{align*}
with the following parameters,
\begin{itemize}
    \item The CRS size is $\poly(n)$, where $n$ is the number of vertices in the graph.
    \item The proof size is $O(n^{c})$, where $c \in (0, 1)$ is a constant. 
\end{itemize}
\end{theorem}

Let $\family{C_x}_{x \in \lang_\YES \cup \lang_\NO}$ be the circuit family that takes the witness, i.e. an isomorphism $\phi$, as input, and verifies if $\phi$ is indeed an isomorphism between $G_1$ and $G_2$.
We will show that there exists a $(2^{\tilde{O}(\sqrt{n})}, \poly(n))$-propositional proof of unsatisfiability for any instance in $\lang_\NO$. Indeed, in \Cref{lemma:babai-proof}, we show that the ``completeness'' of Babai's subexponential time algorithm \cite{Babai80} for the isomorphism problem of strongly regular graphs can be proven using $2^{\tilde{O}(\sqrt{n})}$-length and $\poly(n)$-space propositional proofs.

By \Cref{thm:bounded-space-prop-to-ckt-ext}, there exists a locally unsatisfiable extension of size $2^{\tilde{O}(\sqrt{n})}$ and space $\poly(n)$. Moreover, the extension circuit is $\poly(n)$-locally computable. From \Cref{sec:super-poly-extension}, we obtain a SNARG for $\langISO$ with the parameters claimed in \Cref{thm:SNARGs-Graph-ISO}.

\begin{lemma}\label{lemma:babai-proof}
    Let $\Iso$ be Babai's graph isomorphism algorithm \cite{Babai80} for strongly regular graphs, let $G_1, G_2$ be two strongly regular graphs, and let $R_n( (G_1, G_2), \phi )$ be the verification circuit for the NP-relation $\lang_\YES$. Then the following proportional can be proven by $(2^{\tilde{O}(\sqrt{n})}, \poly(n))$-propositional proofs.
    $$ \prop[ R_n((G_1, G_2), \phi) ], \prop[ \Iso(G_1, G_2) ]  \vdash \out_R \impl \out_\Iso,$$
    where $\prop[ R_n((G_1, G_2), \phi)], \prop[\Iso(G_1, G_2)]$ are the propositional formula representation of the gates and wires in $R, \Iso$, with inputs $G_1, G_2, \phi$ and $G_1, G_2$, respectively, and $\out_R, \out_\Iso$ are the propositional variables representing the output gates of $R$ and $\Iso$, respectively. 
\end{lemma}

To prove the lemma, we first recall Babai's sub-exponential time algorithm for graph isomorphism of strongly regular graphs. At the core of the algorithm is the existence of a \emph{distinguishing set} in strongly regular graphs. We will recall the definition of distinguishing sets in \Cref{def:distinguishing-sets} and states its existence in \Cref{lemma:Babai-distinguish-set}.

\begin{definition}[Distinguishing Sets \cite{Babai80}]\label{def:distinguishing-sets}
    Let $G = (V, E)$ be a graph, a distinguishing set $S$ is a subset of vertices in $V$ such that, for any two different vertices $x, y \in V$,  $\indicator_{S}(x) \neq \indicator_{S}(y)$ or $S \cap \neighbor(x) \neq S \cap \neighbor(y)$, where $\indicator_S$ is the characteristic function for the set $S$.
\end{definition}

\begin{lemma}[\cite{Babai80}]
\label{lemma:Babai-distinguish-set}
    For any strongly regular graphs $G = (V, E)$ of $n$ vertices, there exists a distinguishing set $S \subseteq V$ of size $|S| = \tilde{O}(\sqrt{n})$.
\end{lemma}

We are ready to state Babai's algorithm for the isomorphism of strongly regular graphs.

\medskip
{\bf Input:} Strongly regular graphs $G_1 = (V_1, E_1), G_2 = (V_2, E_2)$ of $n$ vertices.

{\bf Output:} $1$, if $G_1, G_2$ are isomorphic; $0$, otherwise.
\begin{enumerate} 
    \item Find the ``canonical'' labeling of $G_i, i = 1, 2$, as follows. Enumerating an ordered tuple $S = (v_1, v_2, \ldots, v_k)$ of size $k$, where the entries in $S$ are distinct and $k = \tilde{O}(\sqrt{n})$ is an upper bound of the distinguishing set. 
    \begin{enumerate}
        \item Check if $S$ is a distinguishing set. If $S$ is not a distinguishing set, then skip this ordered tuple $S$ and continue to the next ordered tuple. Otherwise, $S$ is a distinguishing set.
        \item For every $x \in V_i \setminus S$, $\neighbor(x) \cap S$ is different for different $x$. Hence, we can sort $V_i \setminus S$ according to $\neighbor(x) \cap S$, as follows. We first define the following vector $\bfu_x = (u_1, \ldots, u_k) \in \bool^k$ for every $x \in V_i \setminus S$. 
        We set $u_i = 1$ if $v_i \in \neighbor(x) \cap S$; Otherwise, we set $u_i = 0$. Then we sort the vertices in $V_i \setminus S$ according to $\family{\bfu_x}_{x \in V_i\setminus S}$. Denote the sorted tuple of vertices as $v_{k+1}, \ldots, v_n$.
        \item Obtain an ordered tuple $(v_1, \ldots, v_k, v_{k+1}, v_n)$ of all the vertices in $V_i$ by concatenating $S$ with the ordered tuple $v_{k+1}, \ldots, v_n$.
        \item Arrange the vertices of $G_i$ according to the ordered tuple $(v_1, \ldots v_n)$, and let $G_S^{(i)}$ be the adjacent matrix of $G_i$.
        \item Let the canonical leveling $\canG_i$ be the adjacent matrix with the minimum lexicographic order among all the $G_S^{(i)}$'s where $S$ is a distinguishing set. \label{Step:Babai-take-min}
    \end{enumerate}
    
    \item If the canonical labeling satisfies $\canG_1 = \canG_2$, output $1$ (the graphs are isomorphic). Otherwise, output $0$ (the graphs are non-isomorphic).
\end{enumerate}

\paragraph{Proof Sketch of \Cref{lemma:babai-proof}.} Now we prove \Cref{lemma:babai-proof}.

\begin{proof}[Proof Sketch of \Cref{lemma:babai-proof}]
    We give a sketch of the claimed $(2^{\tilde{O}(\sqrt{n})}, \poly(n))$-propositional proofs here. We slightly modify the canonical labeling algorithm to also output the ordered tuple $S_i$ such that $G^{(i)}_S = \canG_i$ for $i = 1, 2$. Then we implement the Step~\ref{Step:Babai-take-min} in the above algorithm as a binary tree, where each node takes the lexicographic minimum of its two children. The leaf nodes of the tree are the all possible $G_S^{(i)}$'s.
    Note that the root-to-leaf path of the tree contains $\tilde{O}(\sqrt{n})$ vertices.
    
    \begin{enumerate}
        \item Prove that, if $\phi: G_1 \rightarrow G_2$ is an isomorphism, then $G_{S_1}^{(1)} = G_{\phi(S_1)}^{(2)}$, where $\phi(S_1)$ is defined as follows. Let $S_1 = \family{v_i}_{i\in[k]}$,
        then $\phi(S_1) = \family{\phi(v_i)}_{i \in [k]}$.

        The propositional logic proof for this step has size $\poly(n)$.\label{step:iso-space-proof-1}
        
        \item Prove that $G_{\phi(S_1)}^{(2)} \le \canG_2$, where ``$\le$'' is the comparison in the lexicographic order. Note that the proposition $G_{\phi(S_1)}^{(2)} \le \canG_2$ can be presented as a formula of $S_1, \phi, G_2, \canG_2$. 
        We prove this proposition by enumerating all possible values of $S' = \phi(S_1) \in [n]^k$ and then prove that $G^{(2)}_{S'} \le \canG_2$. 
        
        Note that for every fixed $S' \in [n]^k$, we have a $\tilde{O}(\sqrt{n})$-size propositional proof of $G^{(2)}_{S'} \le \canG_2$. The propositional proof simply contains the root-to-leaf path of the binary tree. In total, this step takes $n^k = 2^{\tilde{O}(\sqrt{n})}$ sizes. But its space is $\poly(k)$, because in each iteration of the enumeration, we only need to keep a counter of $S'$ in the memory.
        \label{step:iso-space-proof-2}

        \item Combining \Cref{step:iso-space-proof-1} and \Cref{step:iso-space-proof-2}, we have proven in propositional logic that $\canG_1 \le \canG_2$. In the rest of the proof, we will show that $\canG_2 \le \canG_1$.
        \label{step:iso-space-proof-3}


        \item We prove in propositional logic that if $\phi: G_1 \rightarrow G_2$ is an isomorphism, then $\phi' = \phi^{-1}$ is also an isomorphism, mapping from $G_2$ to $G_1$.

        The size of the propositional logic proof in this step is $\poly(n)$.
        \label{step:iso-space-proof-4}

        \item We repeat the steps from \Cref{step:iso-space-proof-1} to \Cref{step:iso-space-proof-3}, and prove in propositonal logic that $\canG_2 \le \canG_1$.

        The size and space of the proof in this step is the same as the proofs from \Cref{step:iso-space-proof-1} to \Cref{step:iso-space-proof-3}. Hence, the size is bounded by $2^{\tilde{O}(\sqrt{n})}$ and the space is bounded by $\poly(n)$.
        \label{step:iso-space-proof-5}
        
        \item Finally, we prove in propositional logic that if $\canG_1 = \canG_2$, using \Cref{step:iso-space-proof-3} and \Cref{step:iso-space-proof-5}.

        The size of the proof in this step is $\poly(n)$.
    \end{enumerate}

    The size of the propositional logic proof in each step in the above sketch is $2^{\tilde{O}(\sqrt{n})}$ and the space is $\poly(n)$. Hence, we find an $(2^{\tilde{O}(\sqrt{n})}, \poly(n))$-propositional proof for the ``completeness'' of the graph isomorphism algorithm. This finishes the proof.
\end{proof}

==> impossibility-new.tex <==
\section{Impossibility of Publicly-Verifiable $\SNARG$s for Robust Oracle-Aided Computations}\label{sec:impossibility}

In this section, we prove a lower bound on the oracle-query complexity
of a $\SNARG$ with deterministic public verification and short public
parameters. The lower bound holds even when the computation is
deterministic and the input is fixed before setup.

\begin{theorem}\label{thm:impossibility}
There does not exist a $\SNARG$ with completeness and non-adaptive
soundness for general robust deterministic oracle-aided computations,
with oracle-free setup, deterministic public verification, public
parameters of length $o(n)$, and a verifier making $o(q)$ oracle
queries, where $n$ is the input length and $q$ is the number of oracle
calls made by the computation.
\end{theorem}

Here, non-adaptive soundness means that the adversary fixes its input
before seeing the public parameters. Our argument does not use any bound on the proof length,
and thus holds even for {\em non-succinct} non-interactive arguments.
The computation used below is deterministic, but its oracle queries
may depend on answers to earlier queries.

We prove a more quantitative statement. Let $d$ be the bit length of
the initial oracle answers and the row indices in the computation
below. If the computation makes $q=2N$ oracle calls, the public
parameters have fixed encoded length $m$, and the verifier makes at
most $\ell\leq N/8$ oracle queries, our argument applies whenever
\begin{equation}\label{eq:short-pp-range}
    m+\left\lceil\log_2\max\{\ell,1\}\right\rceil+3\leq d.
\end{equation}
Under these conditions, we obtain a contradiction to completeness or
non-adaptive soundness with constant probability. The false inputs
used in the soundness attack are $1/8$-robust. Taking $d=n$ gives the
theorem and allows public parameters almost as long as the input.
Allowing $d>n$ also gives a lower bound when the public parameters are
longer than the input, as explained below.

\begin{proof}
Let $n=n(\secp)$, $d=d(n)$, and $N=N(n)$, with $n,d,N$ polynomially
bounded in $\secp$, and assume that $N$ is odd. We first give the
construction at a fixed security parameter, and then explain how to
fix one oracle for all security parameters.
We use an oracle with two disjoint types of queries: $\calO(0,i)$
returns a $d$-bit string, and $\calO(1,u,i)$ returns a bit, where
$i\in[N]$ and $u\in\{0,1\}^d$. We refer to
$\bigl(\calO(1,u,1),\ldots,\calO(1,u,N)\bigr)$ as the row indexed by
$u$. The length parameters are included in the query encodings and
are suppressed in the notation; in particular, $d$ is encoded in
unary. These tags separate the queries for different parameter
choices. Outside the current set of tagged queries, all the oracles
below agree with a previously fixed background oracle.

Consider the following deterministic computation on an input
$x\in\{0,1\}^n$. It first reads $\calO(0,1),\ldots,\calO(0,N)$ and
computes
\[
    w=\bigoplus_{i=1}^N\calO(0,i).
\]
It then reads the row indexed by $w$ and outputs its majority:
\[
    C^\calO(x)=\mathsf{Maj}\bigl(
        \calO(1,w,1),\ldots,\calO(1,w,N)\bigr).
\]
The computation ignores the contents of $x$, makes exactly $2N$
oracle calls, and runs in time polynomial in $n,d,N$. We fix the input
$x_0=0^n$ before setup.

Suppose that there exists a $\SNARG$
$\Pi=(\Gen,\mathcal{P},\mathcal{V})$ for this computation, with
oracle-free setup, public parameters of length $m<d$, and a
deterministic verifier making at most $\ell\leq N/8$ oracle
queries.\footnote{For simplicity, we take the public parameters to
have a fixed length. Strings of length at most $m_0$ can be encoded
injectively in $m_0+1$ bits by
$c\mapsto c\,\|\,1\,\|\,0^{m_0-|c|}$. Thus, in the quantitative
bound, $m$ denotes the encoded length.}

The idea is to make every row of the actual oracle mostly zero, so
that every accepting purported execution must contain many incorrect
oracle answers. For each $\crs$, however, we construct another oracle
under which the same fixed input is accepting, and use an honest
proof relative to this oracle. The tricky part is to define one
actual oracle before setup, while ensuring that the verifier is
unlikely to see any difference.

\paragraph{Defining the oracle.}
Sample independently uniform strings
$R_1,\ldots,R_N\in\{0,1\}^d$, an index $J\gets[N]$, a random tape
$r$ for the prover, and an injective affine map
\[
    f:\{0,1\}^m\longrightarrow\{0,1\}^d.
\]
Specifically, take $f(c)=Ac+b$ over $\mathbb{F}_2$, where $A$ is
uniform among the $d\times m$ matrices of full column rank and
$b\gets\{0,1\}^d$ is uniform. Write
$\theta=(f,R_1,\ldots,R_N,J,r)$ for these choices.

For every possible parameter string $\crs$, let
$w_\crs=f(\crs)$ and define
\[
    R_i^\crs=
    \begin{cases}
        R_i, & i\neq J,\\
        w_\crs\oplus\displaystyle\bigoplus_{j\neq J}R_j,
            & i=J.
    \end{cases}
\]
Thus, $\bigoplus_i R_i^\crs=w_\crs$. Let $\calO^+_\crs$ be the oracle
whose initial answers are $R_1^\crs,\ldots,R_N^\crs$, whose row
$w_\crs$ is all ones, and whose other rows are all zeros. Outside
the current set of tagged queries, it uses the background oracle.
All remaining queries are answered with zero. Notice that
$C^{\calO^+_\crs}(x_0)=1$.

Let
\[
    \pi_{\crs,\theta}
    =\mathcal{P}^{\calO^+_\crs}(\crs,x_0;r),
\]
and let $I_{\crs,\theta}\subseteq[N]$ be the positions of row
$w_\crs$ queried by the verifier in the execution
\[
    \mathcal{V}^{\calO^+_\crs}
        (\crs,x_0,\pi_{\crs,\theta}).
\]
We have $|I_{\crs,\theta}|\leq\ell$.\footnote{We truncate all
simulations at fixed polynomial time bounds and retain at most
$\ell$ target-row positions. This does not affect honestly generated
parameters and ensures the stated bound for every parameter string.}

Define the actual oracle by $\calO_\theta(0,i)=R_i$ and
\begin{equation}\label{eq:short-pp-oracle}
    \calO_\theta(1,u,i)=
    \begin{cases}
        1, & \text{if }u=f(c)\text{ for some }c\in\{0,1\}^m
             \text{ and }i\in I_{c,\theta},\\
        0, & \text{otherwise}.
    \end{cases}
\end{equation}
Outside the current set of tagged queries, it uses the same
background oracle; all remaining queries are answered with zero.
Since $f$ is injective, this definition is unambiguous. We emphasize
that it specifies the oracle for every possible parameter string
before the actual $\crs$ is sampled.

\paragraph{Robustness.}
Every row of $\calO_\theta$ contains at most $\ell$ ones, and hence
$C^{\calO_\theta}(x_0)=0$. Consider any accepting purported execution.
Regardless of the answers used in its first $N$ calls, it selects
some row. Since that row contains at most $\ell$ ones, obtaining a
majority of ones requires at least
\[
    \frac{N+1}{2}-\ell\geq\frac{3N}{8}
\]
incorrect answers in the last $N$ calls. There are $2N$ calls in total,
so $C^{\calO_\theta}$ is $1/8$-robust on $x_0$. In fact, the same
argument applies to every input.

\paragraph{The cheating prover.}
The adversary fixes $x_0$ before setup. Given $\crs$, it outputs
$\pi_{\crs,\theta}$. That is, it simulates the honest prover under
$\calO^+_\crs$ using random tape $r$. It answers queries with the
current tags using the explicit definition of $\calO^+_\crs$, and
forwards all other queries to the actual oracle. Once $\theta$ is
fixed, this is a polynomial-size oracle adversary: all the strings
in $\theta$ have polynomial length, and the simulation has
polynomial overhead.

\paragraph{Analysis.}
We first show that the simulated accepting oracle is independent of
$\crs$ in distribution, despite its definition using $\crs$.
Fix $\crs$ and $J=j$. For every tuple
$U=(U_1,\ldots,U_N)$ of $d$-bit strings,
\begin{align*}
    \Pr_{f,R}\bigl[R^\crs=U\mid\crs,J=j\bigr]
    &=\Pr_f\left[f(\crs)=\bigoplus_i U_i\right]
      \cdot\Pr_R\bigl[R_i=U_i\text{ for all }i\neq j\bigr]\\
    &=2^{-d}\cdot2^{-d(N-1)}
     =2^{-dN}.
\end{align*}
Thus, before fixing $\theta$, the tuple $R^\crs$ is uniform and
independent of both $\crs$ and $J$. Moreover, the entire oracle
$\calO^+_\crs$ is determined by this tuple: its initial answers are
$R^\crs$ and its unique all-one row with the current tags is indexed
by their XOR. Since
setup makes no oracle queries, the probability
\begin{equation}\label{eq:short-pp-completeness}
    a=\Pr_{\theta,\,\crs\leftarrow\Gen(1^\secp)}
    \left[
        \mathcal{V}^{\calO^+_\crs}
        (\crs,x_0,\pi_{\crs,\theta})=1
    \right]
\end{equation}
is the average honest-acceptance probability for a distribution of
oracles fixed independently of setup. We use this observation below
to obtain a contradiction from ordinary completeness.

The same argument shows that $J$ is independent of the entire
simulated oracle, proof, and verifier execution. Consequently,
\begin{equation}\label{eq:short-pp-prefix}
    \Pr\bigl[
        \mathcal{V}^{\calO^+_\crs}
        \text{ queries }(0,J)
    \bigr]\leq\frac{\ell}{N}.
\end{equation}
This remains true even if the proof reveals all of $R^\crs$.

It remains to account for queries to rows other than $w_\crs$.
Condition on $\crs,R^\crs,r$, and let $B$ be the set of other rows
with the current tags visited by the simulated verifier. Under this conditioning, its
entire execution is determined and $|B|\leq\ell$. The map $f$ is
still uniform among injective affine maps satisfying
$f(\crs)=w_\crs=\bigoplus_i R_i^\crs$. For each $u\neq w_\crs$,
\[
    \Pr_f\bigl[u\in\operatorname{im}(f)\mid f(\crs)=w_\crs\bigr]
    =\frac{2^m-1}{2^d-1}.
\]
Indeed, conditional on $f(\crs)=w_\crs$, the image is a uniform
$m$-dimensional affine subspace containing $w_\crs$. A union bound
therefore gives
\begin{equation}\label{eq:short-pp-other-rows}
    \Pr\bigl[B\cap\operatorname{im}(f)\neq\emptyset\bigr]
    \leq\ell\frac{2^m-1}{2^d-1}.
\end{equation}

Suppose that neither of the events in
Equations~\eqref{eq:short-pp-prefix} and
\eqref{eq:short-pp-other-rows} occurs. Every answer seen by the
verifier is then unchanged when $\calO^+_\crs$ is replaced by
$\calO_\theta$. The only initial answer that may differ is at $J$,
which is not queried. The queried positions of row $w_\crs$ are
preserved by construction, and every other queried row is outside
$\operatorname{im}(f)$ and therefore remains all zero. Queries with
other tags receive the same background answers. Since the
verifier is deterministic, it follows the same execution and makes
the same decision under both oracles.

Together with Equation~\eqref{eq:short-pp-completeness}, this gives
\begin{equation}\label{eq:short-pp-attack}
\begin{split}
    &\Pr_{\theta,\,\crs\leftarrow\Gen(1^\secp)}
    \left[
        C^{\calO_\theta}(x_0)=0\ \land\
        \mathcal{V}^{\calO_\theta}
        (\crs,x_0,\pi_{\crs,\theta})=1
    \right]\\
    &\hspace{2em}\geq
    a-\frac{\ell}{N}
      -\ell\frac{2^m-1}{2^d-1}.
\end{split}
\end{equation}
Here $\theta$ and $\crs$ are sampled independently. By averaging,
there is a fixed choice $\theta^*$ for which the same lower bound
holds over $\crs$ alone. Thus, for these parameters, setting
$\calO=\calO_{\theta^*}$ gives an oracle fixed before setup and a
polynomial-size cheating prover for the fixed false robust input
$x_0$.

For $m\leq d$, we have
\[
    \frac{2^m-1}{2^d-1}\leq 2^{m-d}.
\]
Thus, Equation~\eqref{eq:short-pp-range}, together with
$\ell\leq N/8$, bounds the two error terms in
Equation~\eqref{eq:short-pp-attack} by $1/4$ in total. Whenever
$a\geq 1/2$, the fixed cheating prover is therefore accepted with
probability at least $1/4$. Taking $d=n\geq\secp$, odd
$N=\Theta(n)$, $m=o(n)$, and $\ell=o(N)$ satisfies these bounds for
all sufficiently large parameters.

\paragraph{Fixing a single oracle.}
To fix one oracle for all security parameters, apply this construction
along a sufficiently sparse increasing sequence
$\secp_1,\secp_2,\ldots$. At each stage, use all previously fixed
answers as the background oracle, and answer every other query
outside the current tags with zero. Choose the next parameters so
that their unary $d$-tag is longer than the worst-case running time
of every capped prover and verifier simulation at all preceding
stages. Later choices then cannot affect any preceding experiment.

At stage $j$, let $a_j$ be the probability in
Equation~\eqref{eq:short-pp-completeness}. If $a_j<1/2$, the
independence argument above implies that there is a fixed accepting
tuple $U$ for which the honest verifier rejects with probability at
least $1/2$, over setup and the honest prover's randomness. Fix the
current answers to be this accepting oracle. Otherwise, the bound
in Equation~\eqref{eq:short-pp-attack} gives a choice $\theta_j$
for which the verifier accepts the fixed false robust input with
probability at least $1/4$. Fix the current answers to be
$\calO_{\theta_j}$.

This defines a single oracle. If the first case occurs infinitely
often, ordinary completeness fails for this oracle. Otherwise, the
second case occurs infinitely often. A polynomial-size adversary
then uses $\theta_j$ as advice at those parameters and performs the
simulation described above, forwarding queries outside the current
tags to the actual oracle. Its input is always fixed before setup,
and its success probability is at least $1/4$ at infinitely many
security parameters. This contradicts non-adaptive soundness.
\end{proof}

\paragraph{Public parameters succinct in $T$.}
The use of $d$-bit row indices, independently of the input length,
also lets us rule out public parameters of length
$\operatorname{poly}(\secp,\log T)$ even when they are not $o(n)$.
For example, consider a fixed machine of the form above with
$d(n)=2^{\lfloor n/2\rfloor}$ and an odd
$N(n)=\Theta(d(n))$. Its time bound can be taken to be
$T(n)=\operatorname{poly}(n)2^n$. For any proposed polynomial bound
on the public-parameter length, take
$n=\lceil a\log_2\secp\rceil$ for a sufficiently large constant
$a$. Then $d$ and $N$ exceed the public-parameter length by a
polynomial factor, while $T$ remains polynomially bounded in
$\secp$. If $\ell=o(N)$, Equation~\eqref{eq:short-pp-range} holds
for sufficiently large parameters. Thus, the same efficient
non-adaptive attack applies. This argument uses a bound on the
public-parameter length, but no bound on the proof length.

\paragraph{The implication for $\IVC$.}
The same lower bound applies to $\IVC$. Modify the computation to
erase its work and oracle tapes, restore its head positions, and
halt at a fixed padded time in a canonical accepting or rejecting
configuration. These additional steps make no oracle queries.
The claimed accepting endpoint, including its time and oracle-call
counters, is then fixed before setup. An $\IVC$ proof for this
endpoint would give a non-interactive argument for the completed
computation with the same public parameters and verifier query
bound, contradicting the result above.


==> intro.tex <==
\section{Introduction}
\label{sec:intro}

 Incrementally verifiable computation (IVC) \cite{} maintains a succinct proof of the correctness of a computation executed, which can be updated as the computation continues:  after each step, a prover updates the proof to certify the current configuration, without retaining or recomputing the preceding execution.   

 In the context of AI safety, the need for incremental verification is particularly compelling for oracle-aided computations. Consider a long-running computation that repeatedly interacts with external sources of information, such as external online databases or experts. It is infeasible to retain its entire execution history, or even reconstruct that history whenever the correctness of its current state must be verified. An IVC scheme for oracle-aided computation would instead allow the computation to carry a succinct certificate of its current configuration, updating this certificate as each new computation step or oracle interaction occurs.  

Unfortunately, oracle access introduces a fundamental obstacle to efficient verification, even for a single completed computation. To illustrate the problem, let us envision the setup.A polynomial-time prover is interacting with  a super-efficient verifier  who both have access to an external oracle, but the super-efficient verifier makes much fewer queries to the oracle. Certifying the correctness of an execution that may depend on many answers of the oracle, requires verifying not only that the computation was executed correctly, but also that the oracle answers claimed to be used  during the computation were in agreement with the underlying oracle. For arbitrary oracles, a single incorrect answer may change the outcome of an otherwise valid computation. A cheating prover can therefore present an execution consistent with an oracle that differs from the true oracle on just one query. Detecting such a discrepancy would require the verifier to check that particular query, and in general may require checking every oracle answer. This difficulty persists even when the computation itself could be efficiently verified via a succinct proof. 

To address this challenge, recent work of Chen, Kalai,, and Xi \cite{}, on  interactive proofs to verify  single (rather than incrementally updatable as we will consider here) oracle-aided computation, restricted its attention to   \textit{robust computations}, in which  changing only a small fraction of the oracle answers will not change the outcome of the computation. 
This property makes it possible, in principle, to detect an incorrect execution by inspecting only a small random sample of its oracle calls. Indeed, \cite{} could show  doubly efficient interactive verification protocols for robust oracle-aided computations. 

In this paper we ask:   can an ongoing computation that \textit{continually consults external oracle} for advice or lookup of facts and expertise, maintain a short and efficiently \textbf{up-datable} proof of its correctness. Achieving oracle aided IVC (even for robust computations) presents a challenge beyond constructing a succinct argument for a completed execution. Whereas a non-incremental prover may use the entire execution transcript to generate its proof,  an incremental prover must update its proof using only the current state and a short maintained certificate. In particular, it must preserve the ability to verify a representative sample of an adaptively growing sequence of oracle calls, even after the earlier queries and answers are no longer available. Moreover, the number of oracle calls is not necessarily known in advance.

\textbf{Our first contribution:} \textbf{The case of robust computations. }

We investigate whether robustness suffices to obtain succinct non-interactive arguments (SNARGs), and ultimately IVC, for oracle-aided computations. 

We first establish a fundamental limitation: robustness alone does not suffice for deterministic publicly verifiable SNARGs with public parameters of length \$o(n)\$ and a verifier making \$o(Q)\$ oracle queries, where \$n\$ is the input length and \$Q\$ is the number of oracle calls. Our impossibility result holds even when the oracle is fixed independently of setup and regardless of proof length. In particular, it rules out publicly verifiable IVC with these parameters. Recall that a SNARG   is a succint \textbf{non-interactive }argument of correctness.

We next show, under the learning with error (LWE) assumption, that if the verifier knows some secret private information, it is possible to construct both SNARGs and IVCs for robust oracle-aided computations. Our construction holds for  bounded-space deterministic and non-deterministic computations, with  $poly(\lambda,S,\log T,1/\epsilon)$ size public parameters, private verification keys, and proofs length where \$\lambda\$ is the security parameter, \$S\$ is the space bound, and \$T\$ is the computation time. Verification requires only \$O(\textbackslash{}lambda\/\textbackslash{}epsilon)\$ oracle queries, independent of the total number of oracle calls. Crucially, the IVC proof can be updated after every computation step without revisiting the execution history or accessing the private verification key.

The main challenge for  the IVC construction is to reconcile incremental proof maintenance with the hidden random sampling needed to exploit robustness. We address this by separating the computation into intervals of ordinary computation and individual oracle calls. Standard IVC techniques certify the computation between oracle calls, while an updatable batch argument maintains a succinct authentication of the growing sequence of oracle-call records. A new quantitative soundness analysis, based on a potential measuring the minimum number of incorrect oracle answers needed to reach a claimed configuration, shows that a small number of hidden oracle checks suffices even against adaptively chosen statements and proofs. The analysis does not assume that locally extracted witnesses arise from a single globally consistent execution.

This result establishes that robust oracle-aided computations can be incrementally verified maintaining succinct proofs and a number of verifier oracle queries independent of the execution length, despite the impossibility of achieving the corresponding deterministic public-verification guarantee.

\textbf{Our second contribution: Public verification through signed oracles.} Private verification, however, is not always sufficient. In many applications, a computation must produce a certificate that can be checked by any interested party, without a secret verification key or continued access to the original oracle. Moreover, robustness can be an unnatural restriction: many important computations depend critically on individual oracle answers, and a single incorrect answer may invalidate the result.

This motivates a different approach. Rather than restricting the sensitivity of the computation to oracle errors, we introduce the notion of a \textit{signed oracle}, which authenticates each query-answer pair using a digital signature. A signed oracle provides a cryptographic certificate of each oracle response, allowing the correctness of oracle interactions to be verified without consulting the oracle itself. Unlike robustness, this assumption places no restriction on how sensitively the computation depends on individual answers.

We next show that, under LWE,  signed oracles enable publicly verifiable SNARGs and IVC for arbitrary oracle-aided computations, without any robustness assumption on the computation, under LWE. Neither setup nor verification requires oracle access, and the public parameters and proofs have length \$poly(\lambda,S,\textbackslash{}log T)\$. 
For deterministic computations with sufficiently short oracle queries and answers, we further obtain fully succinct constructions with public parameters and proofs of length $poly(\lambda,\log T)$, independent of the computation's space complexity.

We note that the signed-oracle model is primarily a conceptual contribution: it identifies a natural authentication mechanism under which the obstruction to public verification can be overcome, even for non-robust computations. Once oracle responses are authenticated, the constructions largely follow established techniques for succinct arguments and incremental verification, augmented with signature checks and an extraction-based soundness argument.

Taken together, our results delineate two complementary possibilities for incrementally verifiable oracle-aided computation. Robustness enables succinct incremental verification of unauthenticated oracle computations using private verification and a small number of oracle queries; signed oracles enable public, oracle-free verification even for non-robust computations. The former requires new techniques for incrementally maintaining and privately checking a growing oracle transcript, while the latter provides a general conceptual framework for publicly verifiable computation that relies on authenticated external information.


%We study two ways to overcome it. The first imposes structure on the oracle: each answer is accompanied by a signature authenticating the query–answer pair.  The second imposes structure on the computation: we restrict our attention to computations for which producing an incorrect result requires a substantial fraction of the oracle answers to be wrong.  These results extend the scope of IVC along two complementary directions.
%In more detail, we construct succinct non-interactive arguments (SNARGs) and IVC schemes in both settings under the \textit{Learning With Errors} (LWE) assumption. Indeed, we first develop succinct non-interactive arguments (SNARGs) in each setting and then use it as a tool to construct incremental schemes  that preserve their verification guarantees throughout the computation. The two settings lead to different verification guarantees.  
%\begin{itemize}
%Signed answers permit public verification without access to the oracle.
%Robustness permits verification with few oracle queries, using a private verification key. We also prove a lower bound showing that robustness alone cannot, in general, provide the same  guarantee with deterministic public verification and short public parameters. 
%\end{itemize}

\textbf{1.1 Our Results in a bit more detail}

Throughout, let $\secp$ denote the security parameter, n the input length, and T, S, and Q the time, space, and oracle-query bounds. Our constructions support deterministic and non-deterministic oracle-aided computations and achieve adaptive soundness: the adversary may choose the statement and proof after seeing the public parameters. The underlying oracle is fixed independently of setup, and all cryptographic assumptions are required to hold even given access to it.

\textbf{Robust computations with arbitrary oracles.}  We require  that the computation be robust against incorrect oracle answers. On a false input, every purported accepting execution that follows the ordinary transition rules must contain an ϵ-fraction of incorrect oracle answers. Thus, an incorrect conclusion cannot be explained by only a few erroneous answers.

For such computations, we construct privately verifiable SNARGs and IVC schemes with public parameters, private verification keys, and proofs of length poly(\lambda, S,\log T,1\/\epsilon). Setup makes no oracle calls, and verification makes only $O(\lambda\/\epsilon)$ oracle calls. Proof updates do not require the private verification key or access to the preceding execution. These constructions assume sub-exponential hardness of LWE.

\textbf{Extending to IVC. }Robustness must apply to the current configuration being certified. Namely, if an execution reaches an incorrect claimed configuration must contain an ϵ-fraction of incorrect oracle answers. Robustness of the final output alone need not imply this property for intermediate configurations. For an accepting terminal configuration on a robust false instance, the required condition follows from the robustness of the computation.

For deterministic computations, we further remove the dependence of proof and public-parameter length on the space bound. When oracle queries and answers have length poly(λ,logT), these lengths become poly(λ,logT). The general constructions use sub-exponential hardness of LWE; in the deterministic signed-oracle setting with polynomially bounded computation time, polynomial hardness suffices.

\textbf{Signed oracles.} Suppose that the oracle returns, with each answer a to a query u, a digital signature authenticating (u,a). We construct publicly verifiable SNARGs and IVC schemes whose public parameters and proofs have length  poly(\lambda, S,\log T). Neither setup nor verification requires access to the oracle, and no robustness assumption is needed. In the incremental setting, the prover updates its proof after each computation step without revisiting the preceding execution.



\textbf{A limitation of public verification.}

We complement these constructions with an impossibility result. For arbitrary oracles, robustness alone does not suffice to obtain SNARGs or IVC with deterministic public verification, public parameters of length o(n), and o(Q) verifier oracle queries. The lower bound holds even when the oracle is fixed independently of setup and regardless of proof length. Within these bounds, the private verification key in our robust construction addresses a genuine limitation of public verification.

\textbf{1.2 Related Work}

\textbf{Verification of oracle-aided computations.}

Our work builds on the recent study of efficient verification for oracle-aided computations. Chen, Kalai, and Xi [?] construct doubly-efficient interactive proofs and arguments for oracle-aided computations under additional structure on the computation or the oracle. In particular, they give protocols for robust computations, where the output is insensitive to a small fraction of incorrect oracle answers, as well as for computations with access to a low-degree oracle. We study non-interactive and incremental verification. For robust computations, we construct privately verifiable SNARGs and IVC schemes whose verifiers make few oracle queries.

\textbf{Signed oracles.}

Chiesa and Tromer [?] introduced a signed random-oracle model, where oracle answers are random and accompanied by signatures, and used it to construct short non-interactive arguments and proof-carrying data, a generalization of IVC. More recently, Maller, Mohnblatt, and Zapico [?] introduced the open-and-sign random-oracle model and constructed IVC in this model. Both works rely on an idealized random-oracle functionality. Our signed-oracle results accommodate arbitrary authenticated oracle answers under LWE, with oracle-free setup and verification.

\textbf{Incremental verification with oracle access.}

The distinction between proving a completed oracle-aided computation and maintaining a proof incrementally is central to our work. Beyond the signed-oracle setting above, our robust-oracle construction addresses the challenge of maintaining a succinct proof that supports hidden checks of an evolving sequence of unauthenticated oracle answers. It combines incremental certification of ordinary computation with updatable aggregation of oracle-call records, preserving the quantitative soundness guarantee as the execution grows. Our constructions build on the updatable batch arguments of Aldema Tshuva and Oshman [TO26]; the additional analysis establishes how their local guarantees can certify authenticated oracle answers or support hidden oracle checks under robustness.

\textbf{1.3 Paper Organization}

Section 2 gives a technical overview. Section 3 recalls the cryptographic primitives, and Section 4 defines oracle-aided computation and robust verification. Section 5 constructs privately verifiable SNARGs for robust computations; Section 6 establishes the public-verification lower bound. Section 7 constructs publicly verifiable SNARGs for signed oracles, including the fully succinct deterministic variant. Section 8 develops our IVC definitions and constructions for both settings.






==> temp-signed.tex <==
------------


For signed oracles, the construction is somewhat simple, and can use any $\SNARG$-to-$\IVC$ construction, as long as the $\SNARG$ has an  additional local extraction property.  A signature on an oracle query-answer pair can be viewed as a witness certifying the corresponding oracle transition.  Note that valid witnesses exist even for false claims; i.e., ones that are inconsistent with the oracle. Namely, even for an incorrect answer $a\neq O(u)$, there exists a
valid signature on $(u,a)$ under the oracle's signing key. but these signatures (i.e., witnesses) are hard to find, as finding them requires forging a signature.  Therefore, ordinary soundness is not sufficient, and we need $\SNARG$s that are somewhere extractable, i.e., that from an accepting proof for such a transition we can \emph{extract} the signature, and thereby obtain a
forgery.  Thus, we require the underlying $\SNARG$
to satisfy an appropriate somewhere-extraction,
property.  We then use the updatable argument machinery of Aldema
Tshuva and Oshman~\cite{AldemaTshuvaO26} to lift this locally
extractable $\SNARG$ to the incremental setting.

% For robust oracle-aided computations,
% on the other hand, verification must remain private: the verifier needs
% to check a few oracle answers using hidden locations.  In this case we
% use the updatable hash-and-$\BARG$ underlying the same transformation,
% but perform the oracle checks only at the final private verification.






We first consider the signed-oracle setting of \Cref{sec:signed-oracles}.  Recall that
the signed oracle returns
\[
O_{\mathsf{sig}}(u)=(a,\sigma),
\]
where 
\[a=O(u)~~\mbox{ and }~~
\mathsf{Sig.Verify}(\vk,(u,a),\sigma)=1.\]


The main observation is that, once oracle answers are signed, an oracle
transition can be verified by an ordinary, oracle-free computation.
Namely, consider a transition from configuration $C$ to configuration
$C'$.  If this is an ordinary transition, we simply check that it is a
valid transition of $M$.  If this is an oracle transition with query
$u$ and purported answer $a$, the witness additionally contains a
signature $\sigma$, and we check
\[
\mathsf{Sig.Verify}(\vk,(u,a),\sigma)=1.
\]
Thus, signatures turn oracle transitions into ordinary locally
verifiable transitions.

Formally, define the oracle-free one-step relation
$R_{\mathsf{sig}}$ as follows.  A statement consists of a tuple 
\[
D=(t,C,C'),
\]
where $C,C'$ are purported consecutive configurations at time $t$.
A witness certifies that either:
\begin{enumerate}
\item $C\rightarrow C'$ is a valid ordinary transition; or
\item $C\rightarrow C'$ is a valid purported oracle transition,
with query $u$ and answer $a$, together with a signature $\sigma$
such that
\[
\mathsf{Sig.Verify}(\vk,(u,a),\sigma)=1.
\]
\end{enumerate}
Notice that neither $R_{\mathsf{sig}}$ nor the consistency relation
queries the oracle.  Moreover, given a genuine execution of $M^O$,
the prover can obtain all the necessary witnesses using
$O_{\mathsf{sig}}$.

We can now apply the generic $\SNARG$-to-$\IVC$ transformation
of~\cite{AldemaTshuvaO26}.  Equivalently, one may view the construction
as maintaining an updatable proof for the sequence of transition
records above.









\begin{theorem}
\label{thm}
Let $M$ be a time-$T$, space-$S$ oracle-aided machine, and let
$O_{\mathsf{sig}}$ be a signed oracle as in \Cref{def:signed-oracle}.
There exists a publicly verifiable $\IVC$ scheme for executions of
$M^O$ with adaptive soundness.  Setup and verification make no
oracle calls.

The public parameters and proof have length
$\poly(\lambda,S,\log T)$,
and proof update and verification take time
$\poly(n,\lambda,S,\log T)$.
The prover makes exactly the oracle calls made by the underlying
execution.

The construction is secure assuming the security of the underlying updatable hash-and-$\BARG$ and existential unforgeability of the signature
scheme, even given access to $O$.
\end{theorem}

\begin{proof}
Completeness and efficiency follow directly from the completeness and
efficiency of the updatable $\IVC$ transformation.  It remains to relate
soundness for the signed-transition relation to soundness for the underlying oracle computation.

Suppose that an adversary produces an accepting $\IVC$ proof for a configuration $C_t$ that is not reachable after $t$ steps of $M^O$.
Except with negligible probability, the consistency and local
soundness properties of the underlying UpBARG imply that the committed
transition records describe a consistent purported execution
$C_0,C_1,\ldots,C_t$, 
starting from the prescribed initial configuration and ending at
$C_t$, where every ordinary transition is valid and every purported
oracle transition carries a verifying signature.

Since $C_t$ is not reachable under the real oracle $O$, at least one
oracle transition in this purported execution uses a query-answer pair
$(u,a)$ for which
$a\neq O(u)$.
We show that such an accepting proof yields a forgery.

Generate the $\mathsf{UpBARG}$ parameters in trapdoor mode with a uniformly
random hidden transition index $j\in[t]$.  By index hiding, this
changes the adversary's success probability by at most a negligible
amount.  From an accepting proof, extract the $j$th transition and its
witness.  With probability at least $1/t$, the extracted transition is
one of the incorrect oracle transitions.  In this case extraction gives
$(u,a,\sigma)$ such that
\[
a\ne O(u)
\qquad\text{and}\qquad
\mathsf{Sig.Verify}(\vk,(u,a),\sigma)=1.
\]
On the other hand, every signature obtained while simulating
$O_{\mathsf{sig}}$ was on a pair $(v,O(v))$.  Thus $(u,a)$ was never
submitted to the signing oracle, and $\sigma$ is a valid forgery.

For polynomially bounded $T$, a $1/T$ loss preserves
non-negligibility.  For larger $T$, we require the corresponding
security against $\poly(T)$-time adversaries with error negligible in
$T$, as in the preceding sections.
\end{proof}

\paragraph{Fully succinct deterministic computations.}
For deterministic computations we may use the compressed configurations
from \Cref{sec:short-signed-oracles}.  In particular, the work tape is represented by its
hash, and every local modification is checked using
$\mathsf{HT.VerifyUpdate}$.  Thus a one-step statement and witness have
length $\poly(\lambda,\log T)$.
Applying the same lifting gives public parameters and $\IVC$ proofs of length $\poly(\lambda,\log T)$, and verification time $n\cdot\poly(\lambda,\log T)$.
The same modification as in Remark~31 handles long queries and
answers by having the oracle sign their hashes.

